PLAID: Supporting Computing Instructors to Identify Domain-Specific Programming Plans at Scale

Pedagogical approaches focusing on stereotypical code solutions, known as programming plans, can increase problem-solving ability and motivate diverse learners. However, plan-focused pedagogies are rarely used beyond introductory programming. Our formative study (N=10 educators) showed that identifying plans is a tedious process. To advance plan-focused pedagogies in application-focused domains, we created an LLM-powered pipeline that automates the effortful parts of educators' plan identification process by providing use-case-driven program examples and candidate plans. In design workshops (N=7 educators), we identified design goals to maximize instructors' efficiency in plan identification by optimizing interaction with this LLM-generated content. Our resulting tool, PLAID, enables instructors to access a corpus of relevant programs to inspire plan identification, compare code snippets to assist plan refinement, and facilitates them in structuring code snippets into plans. We evaluated PLAID in a within-subjects user study (N=12 educators) and found that PLAID led to lower cognitive demand and increased productivity compared to the state-of-the-art. Educators found PLAID beneficial for generating instructional material. Thus, our findings suggest that human-in-the-loop approaches hold promise for supporting plan-focused pedagogies at scale.

==> parking-lot-text/discussion-study1.tex <==
\subsection{LLMs May Provide Opportunities to Support Programming Plan Identification}
\label{sec:opportunities}
% \begin{figure*}
% \centering
% \includegraphics[width=\textwidth]{img/design.png}
% \caption{A proposed sociotechnical plan identification process that mirrors educators' current plan identification procedures while leveraging both human expertise and automated processing for improved efficiency.}
% \label{fig:design}
%   % \Description{This diagram summarizes the proposed sociotechnical plan identification process. The first box represent the candidate plan identification stage where plans are created based on common code sequences, from literature, or from scratch. There is an arrow that originates from this box to the next box that represents the plan refinement stage showing the successive steps. In the plan refinement stage, we modify the abstraction level of plans and receive automatic and crowd-sourced feedback on metrics. This box has a self-loop arrow representing that it is an iterative process until goal is reached. Then, there is an arrow pointing to a plan library symbolizing that a collection of candidate plans has been created. The last arrow from the plan refinement box is to the last box representing the plan elimination stage. At this stage, if the candidate plan does not reach acceptable metrics or does not meet learning goals, it is discarded.}
% \end{figure*}

By providing a more precise understanding of how plan identification is currently performed by educators, as well as the barriers in the current process of plan identification,
% as well as an understanding of several opportunities for improving the efficiency of the plan identification process, 
our interviews highlighted opportunities to leverage generative AI tools like ChatGPT for improving educators' process for plan identification. 
%% KC other thoughts
%
% Our formative study established that a review of practice is a key part of the plan identification. However, reviewing this practice can be time-consuming and tedious. In addition, common code patterns aren't the only important part of programming plans. Educators look for other pieces of information that help students translate the programming plan into practice.
% They use literature. They like a place to start from.
% By getting examples ready and organized, we may be able to improve and speed up the process of programming plan identification. 
% To investigate the feasibility of this plan, we attempt to generate 
% 

% This new processes mirror the stages of educators' current plan identification procedures, while leveraging both distributed human expertise and automated processing. We describe each of these avenues
% % stage of this process 
% below and present a summary in Figure~\ref{fig:design}.

% \subsection{Some Plan Structures Better Support Automated Metrics}

% % take a stance
% % We need code in plans to better find the level of abstraction. In plans with just natural language description, it would be difficult to measure the level of abstraction

% \edit{To allow educators and developers to work together, the system must use a consistent plan definition which includes choosing the necessary plan components that best meet the learning goals of the intended audience. We believe that choosing a programming plan definition where plans are defined in code and where plans have changeable areas will best facilitate automated processes that draw on pools of code examples.}

% \subsection{Choice of Plan components and Perspective}

% To allow educators and developers to working together, the system must use a consistent plan definition. Designers of plan identification systems should choose from the list of components (Section~\ref{sec:components}). We believe that choosing a programming plan definition where plans are defined in code and where plans have changeable areas will best facilitate automated processes that draw on pools of code examples.

% Implications for the choice of plan components


%Based on , we believe that a plan definition that uses a solution in code rather than pseudocode or natural language (Section ~\ref{}) presents more opportunities to partially automate the plan identification process because it allows systems to take advantage of the data in existing code repositories, like GitHub or StackOverflow. Further, we believe that the plan representation in a plan identification system should include specific changeable areas (Section~\ref{}), as it enables automatic calculation of the abstraction level . This idea is further explained below in Section~\ref{}.
 
% \subsubsection{Opportunities to generate candidate plans} % Creation stage

% \subsubsection{Opportunity to Involve AI or Data Mining Tools}
% \textit{``Since it learns from so many, it probably has already kind of done the synthesis itself,''} reasoned P6. P6 also suggested that 

A key challenge mentioned by our participants was how plan identification requires a lengthy and tedious process where the instructor needs to get familiar with many example programs for the domain they are working in. The time-consuming nature of creating a representative, general-purpose programming plan from many examples slows the process of plan identification for educators.
% Reflecting instructors' experiences with plan identification, there are multiple avenues to introduce candidate plans into a system in a way that accelerates the process of plan identification: those that automate the process and those that draw on past work or an educator or programmer's expertise. 
% Some of our educators mentioned that using emerging AI tools like GitHub Co-Pilot (P6) or ChatGPT (P7) to generate solutions could help in plan identification.
In order to support the challenging process of identifying common examples, a plan identification system can \textit{generate candidate plans} by searching relevant pools of code for common pieces of code.
% ~\cite{haggis_code_similarity}, or by prompting a large language model for examples from a particular domain. 
Large language models, which are trained on large corpora of code and include data from many example programs, have been shown to perform reasonably well on code generation and interpretation tasks~\cite{juryEvaluatingLLMgeneratedWorked2024a, finnie-ansleyRobotsAreComing2022}. Thus, LLMs may be able to provide a starting point for instructors by presenting them with potential plan candidates. %with all components that meet the success metrics. %by generating initial plan candidates, including solution code and explanations.

% The user can specify the topics they are interested in identifying programming plans for, and the system could then suggest relevant code corpuses drawn from online code repositories (i.e., Github, Stackoverflow) or instructional materials. As educators vary in their beliefs about the type of practice that plans should represent, users should have the ability to limit the code pools used for candidate generation to those by certain types of authors or another measure of quality.

%\edit{Our participants suggested using emerging AI tools to ask for solutions to the same problems in different contexts and then evaluate code similarity to search for plans.}

% Another method of candidate plan generation could draw on the instructor's current insight. As some instructors prefer to design their own plans, plan identification systems should include the possibility for users to create a candidate plan from their own intuition. %This process of course depends on a user's programming expertise.

% Finally, as some of the educators we interviewed found plans from the literature important in their own plan identification process, systems could allow users to search the existing plan literature as well as programming plans created by other users.

% \subsection{Opportunities to support plan refinement} %Refinement stage

% \subsubsection{Opportunity for Automated Metrics for Abstraction, Commonality, and Usability}
% We found that plan refinement is an crucial stage in educators' plan identification process, but also an area where educators face challenges as they struggle to find the right balance between a plan's frequency in practice (commonality), ease of use (usability), and appropriateness for their learner population. The process of plan identification could become more efficient if educators could receive quicker and clearer feedback about how their candidate plans measure up in each of these characteristics. 
%evaluating the metrics of plan quality that instructors value could be automated or crowd-sourced.} 

% With automated metrics of commonality,  usability, and level of abstraction, the feedback loop that educators undergo as they search for the right version of their programming plan could be shortened. Such automated metrics may be possible, if the right plan components are available. If programming plans are represented in a format that includes their programming language code, a system could search relevant code repositories for similar code in order to provide a measure of a plan's \textit{commonality}. If the system represents programming plans not only in code but also with changeable areas (see Section~\ref{sec:changeable}), then the system can infer the level of abstraction based on what percentage of the plan consists of changeable areas, as well as the complexity of typical code in the changeable areas.

% To measure usability, which is the ease with which learners can modify and apply the plan, code comparison with a relevant corpus may not yield much insight. However, it may be possible to get learners involved through a learnersourcing~\cite{weir2015learnersourcing} activity. The system could connect with novice programmers at the appropriate level and give them an automated task to implement the candidate plan. Based on the correctness of this activity, it could provide a metric for usability.

%\edit{If educators could quickly understand how changes to the programming plan they are refining affect the metrics that they care about, it may increase the efficiency of the plan identification process.}

% During the refinement stage of a plan identification system, instructors can edit the candidate plan with the goal of balancing the metrics of commonality, usability, and level of abstraction to values within their desired thresholds. As some instructors value some metrics more than others, users should have the ability to modify the acceptable ranges for each of these metrics. 

% As instructors add or remove changeable areas to their plan, they receive feedback from the automated metric values. Instructors' expertise is particularly relevant in the refinement stage, as they not only rely on the system for information about the value of their candidate plan, but also judge its appropriateness themselves. 

% Automated metrics may not completely replace the benefits educators gain from conversations with their peers. In our interviews, we learned that the educators we worked with had extensive conversations about plan identification during their process (see Section~\ref{sec:discussions}). Conversations between educators can also be supported in a plan identification system, perhaps through chats, a commenting system, or suggestions for plan changes.
%as the instructors we interviewed were clear that these conversations led to improved plan identification outcomes. These reflections on the quality of the plans and conversations can occur through chats and even spontaneous video calls enabled by the system. }

% \subsubsection{Opportunities to support plan identification in domains unfamiliar to educators} %Refinement stage

Moreover, LLMs may be able to allow instructors to identify plans in unfamiliar domains by presenting them with plan candidates from those domains. 
% Enabling direct collaboration between instructors and large language models could allow for easier identification of programming plans in specific application areas, as the LLM can suggest plans from the large amount of data it was trained on,
% personal expertise or during a guided think-aloud
A system that acts as a collaborator for the instructor might expedite the domain-specific plan identification process significantly. Through such a system, an instructor can obtain initial plan candidates in any domain and refine those plans such that they are appropriate for learners. This approach could make it possible to greatly expand the number of domains where the plans can be used for instruction, as it would no longer require a single person to have both instruction expertise and in-depth domain knowledge. 

% Based on our findings, it's important to combine programming expertise with instructional expertise 
% contribute in ways that make use of their particular strengths 
% (see Section~\ref{sec:individual-design}). 
% For experts in the programming domain, a system could encourage their participation in the candidate plan stage in particular. This may include sharing information about a plan's commonality in a particular domain, as well as information about the intent of a candidate plans. 
% The LLM could contribute to the candidate plan stage in particular. Then, educators may become involved in the plan refinement stage, particularly as they are better positioned to judge how understandable plan components are for the relevant learner audience.

% \subsubsection{Opportunity for Facilitating Discussions Between Educators}


%\subsection{Elimination stage}

%Finally, not all candidate plans will make it into the final plan library. If instructors cannot balance the metrics for a particular plan to acceptable values, or, if the instructors believe that the plan doesn't meet their learning goals, they can remove the plan from consideration. 


==> parking-lot-text/discussion-study2.tex <==
\section{Discussion}

In this section, we address RQ2: \textit{How can LLMs (e.g. ChatGPT) support the identification of domain-specific plans?} 
%With the results of our mixed methods study, we are able to identify the strengths of supporting the plan identification process with LLMs while noting its shortcomings.

% Component generation
We found that our ChatGPT pipeline can reliably generate common domain-specific code. 
%It performs well on code generation tasks, i.e. generating the solution component of a plan, as evident from the 
Our quantitative and qualitative evaluation showed that generated plan solutions were almost entirely syntactically valid (see Section~\ref{sec:quant_accuracy} and Section~\ref{sec:qual_components}). 
In addition, the generated code is representative of actual practice (Section~\ref{sec:quant_commonality}), as shown by similarity to a reference set of plans validated by experts, and comparable similarity to Github files from the same domain (Section~\ref{sec:commonality}). Moreover, accounting from the similar number of distinct methods covered in the two datasets, we infer that ChatGPT can generate plans that capture a variety of use cases in the domain (Section~\ref{sec:quant_usability}). Furthermore, the complexity of the generated code appears to be similar to those generated by instructors with domain expertise, indicating that the generated examples can be appropriate for novices (Section~\ref{sec:quant_learners_appropriateness}). 
Overall, using LLMs for early phases in plan identification by generating common examples and recognizing candidates is a promising avenue.

However, our approach is not consistently able to describe the code appropriately for learners.
It especially falls short on code interpretation, namely, generating other components of a plan such as names and goals. A number of its generated responses were either overly general or overstating what the code achieved (see Section~\ref{sec:qual_components}). This might reflect the existing challenges for LLMs on in-context learning tasks, observed by prior work~\cite{llms_hard_incontext_learning}.
In addition, ChatGPT sometimes generated technical jargon in the names and goals (see~\ref{sec:qual_characteristics}), which makes those plan components unsatisfactory for novice learners. However, despite these pitfalls, the generated plan components were somewhat accurate, implying that they may be appropriate starting points for instructors to refine.

%These findings suggest the role that LLMs can best play in domain-specific plan identification: they can generate candidate plans, however, they lack the capability to create plans that fully meet instructors' desired characteristics. 

We present suggestive evidence that using LLMs to generate candidate plans as a part of a plan generation pipeline could reduce the tedium in the identification process by eliminating the need for instructors to view programs or perform a literature review (Section~\ref{sec:viewing-programs} and Section~\ref{sec:lit-review}) prior to creating plans. Instead, LLMs could provide instructors with candidate plans that they would modify for their learner audience to ensure that the explanatory components are accurate and reasonable. A promising direction for the design of an automated plan identification system is to foster collaboration between an LLM and instructors in order to scale domain-specific plan identification. 
%that allows the instructor to refine the generated candidate plans to meet their learner's goals. 

% ...support instructors through simulating a collaborative process, where the LLM presents initial candidates and the instructor can modify and refine the candidates for their learning goals

% components/ accuracy
% name and goal
    % it seems to perform well on code generation (both qual and quant) but not as well on interpretating what the code does (qual).
%     Evidence on generation: quant similarity to existing plans
%     Related evidence: changeable areas not accurate, goals needed work (from qual)
% solution
    % accurate
% changeable areas
    % accurate yet not quality worthy

    % appropriateness to learning goals - not a metric that can be translated for llms
    
% bigger picture
% can generate quality candidate plans but not the final plans
% needs instructor feedback

% Instructors are still needed in the loop to ensure that explanatory components are correct, and to . A reasonable number were partially correct. 


% Which part of the plan identification process can be automated with LLMs?

% LLMS have the potential to replace the example search and literature review part. + supporting the instructor in domain expertise (by having more variety)

%This section can answer RQ2: How can tools for explaining and generating code
%(e.g. ChatGPT) support the identification of domain-specific plans?




==> parking-lot-text/discussion.tex <==
\section{Discussion}

% Next we summarize the challenges and opportunities in plan identification based on our interview findings, and 


In the prior section, we identified the \textit{components, characteristics, and challenges relevant for the plan identification process}. 
This section focuses on the implications of those results.
% Our findings shed light on the ways that instructors who identify programming plans for educational purposes address inherent difficulties in the plan identification process. 
% In this section, we reflect on the nature of the challenges in plan identification

%%%%
% 1. Translating Values to Metrics
% only use the term metrics for when values can be observed through measurable changes in the code


% ## concrete concepts
%% > Definitions
% ## how to measure the concepts based on code features
%% > Comprehensive look at the balance between plan value
%% > How to actually calculate plan metrics


% ## Plan structures


% Plan identification requires instructor and programing expertise.



% The plan identification procress is iterative and collaborative
%5 In order to balance the tradeoffs
% - Discussion
% - Back and forth between creation and discussion


%%%%%

% \subsection{Educators Must Balance a Variety of Interconnected Values During Plan Identification}

% % \begin{figure}
% % \centering
% % \includegraphics[width=0.5\textwidth]{img/metrics-balance.png}
% % \caption{Relationships between the characteristics educators value when judging quality of programming plans for instruction}.
% % \label{fig:metrics}
% %   % \Description{A circle in the center for representing the abstraction level. A circle on the top-left for representing commonality. An arrow from the abstraction level to commonality with a plus sign to say that as the abstraction level of a plan increases, it becomes more common and hence establish a positive relationship between these metrics. A circle at the bottom-left expressing usability. An arrow from the abstraction level circle to usability with a negative sign indicating that as abstraction level increases, the plans become less usable. A two-way arrow with a plus sign between commonality and usability to indicate that as usability increases, the plans become more common and vice-versa. Another circle on the center-right for determining the appropriateness of the plan for beginners. An arrow from abstraction level to appropriateness for beginners with a negative sign to say that as plans become more abstract, plans become less appropriate for beginners.}
% % \end{figure}

% % describe the triangle of abstraction level in detail
% % tie it back into the previous section
% Based the findings presented in Section \ref{sec:abstraction}, the right level of abstraction was a key characteristic that helped educators determine the quality of a plan. In Section \ref{sec:challenges_abstraction}, we also acknowledge that creating a suitable level of abstraction was a challenge that most of our participants encountered. Educators identifying plans aren't the only ones to face this challenge. In their study of a system for capturing developers' programming strategy knowledge, Arab et al. found that developers had difficulty ``finding the right scope for their strategy'' to share with others~\cite{Arab_StartegySharingSystem_CHI-2022}.

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{img/new-balance.png}
% \caption{Relationships between the characteristics educators value when judging quality of programming plans for instruction.}
% \label{fig:metrics}
%   % \Description{A circle in the center for representing the abstraction level. A circle on the top-left for representing commonality. An arrow from the abstraction level to commonality with a plus sign to say that as the abstraction level of a plan increases, it becomes more common and hence establish a positive relationship between these metrics. A circle at the bottom-left expressing usability. An arrow from the abstraction level circle to usability with a negative sign indicating that as abstraction level increases, the plans become less usable. A two-way arrow with a plus sign between commonality and usability to indicate that as usability increases, the plans become more common and vice-versa. Another circle on the center-right for determining the appropriateness of the plan for beginners. An arrow from abstraction level to appropriateness for beginners with a negative sign to say that as plans become more abstract, plans become less appropriate for beginners.}
% \end{figure}

% Synthesizing our interviewees' responses yields insight into why finding that correct level of abstraction is so difficult: A plan's level of abstraction directly impacts three other desired characteristics, some positively and some negatively (see Figure~\ref{fig:metrics}).  In essence, plan identifiers are performing a balancing act between a plan's commonality, usability, and appropriateness for their students.

% Abstraction level has a direct connection with the \textit{commonality} of a plan. When a plan is more general, it will be seen in practice more often. However, abstraction level has an inverse relationship with how \textit{usable} a plan is. The less specifically a plan is defined, the more interpretation a programmer needs to use to put the plan into use. For instance, with a more abstract plan%(e.g., the bottom plan in Figure~\ref{fig:abstraction})
% , programmers have to make more implementation decisions on their own when they put the plan into practice.

% % this probably needs more unpacking, it makes sense for me but a new reader might not understand this
% %% This is kinda confusing, so I commented out for now
% %\edit{Commonality and usability also have a positive relationship. If a plan is more usable, then it is seen in practice more often and thus it can be termed common. Similarly, the more common a plan is, it can be used in more contexts and thus is more usable.}

% The level of abstraction of a plan has a negative relationship with how appropriate it is for beginners, an important concern for educators specifically. While learners can benefit from instruction about abstract principles~\cite{doi:10.3102/0013189X025004005}, novices have more difficulty applying more abstract representations~\cite{kaminski2006children}. Novices have less familiarity with programming, and therefore programs that an expert sees as similar may be seen as distinct by the novice.
% % a higher level of abstraction makes the programming plan less appropriate for beginners 
% %\edit{due to the prior conceptual background needed to understand them. To illustrate with an example, from Figure 3, if a novice is presented with the third plan (goal: make a selection), it will be challenging for them to understand the structure and purpose of the plan. However, if the same novice is presented with the first plan (goal: validate for equality), it would prove to be less intense because of the amount of scaffolding that comes with the plan.}





% % to determine the desired level of each metric based on their target audience. A more experienced audience may be comfortable with more abstract plans and the educators can focus more on finding a common ground with respect to the other metrics, however, when creating plans for apprentices, focusing on learning goals might be more important than others.

% % i don't think this fits here anymore
% % disbursing it to other sections
%  % The process of plan identification could become more efficient if evaluating the metrics of plan quality that instructors value could be automated or crowdsourced. The instructors we interviewed noted that many of their discussions were about whether plan candidates met their measures of plan quality, particularly the correct level of abstraction. If educators could quickly understand how changes to the programming plan they are refining affect the metrics that they care about, it may increase the efficiency of the plan identification process.
 
% % \subsection{The Plan Identification Process is Iterative and Benefits From Feedback}
% % Iterative — it is, but why. Collaborative and discussion to balance metrics and address challenges

% % introducing the section
% % From the interview study, we find that having discussions with colleagues and other researchers was a key component of our participants' plan identification process. Based on the findings in Section \ref{sec:discussions}, the discussions were often regarding identifying plans, refining them, or making decisions to eliminate them, if necessary.

% % % maybe rephrase later
% % Our interviewees collaboratively used their expertise and resources to look at the large search space for code and identify candidate plans. This collaborative effort helped them address the challenge of choosing plans from practice since each of them identified their own plans and then deliberated upon how to translate code into a programming plan for learners with the necessary components.

% % The instructors also noted that many of their discussions were about plan properties and whether plan candidates met their measures of plan quality, particularly the correct level of abstraction. We believe that these discussions helped them address the challenges they faced to identify the suitable abstraction level that fit the learning goals of their audience. Our participants used their experience to inform their judgment of the characteristics described in the previous section. With their pooled expertise, they were able to balance those values and make decisions about the candidate plans.
% % \edit{In the refinement discussions, our interviewees highlighted that they deliberated about plan properties and plan quality. We believe that such discussions helped them address the challenge of finding the suitable level of abstraction that fit the learning goals of their audience.}




\subsection{Plan Identification for Education Requires More Than Finding Common Pieces of Code}

% findings new programming plans may require both these expertise
% we have evidence from the new domain ques from the interview

% overview
As we note in Section \ref{sec:individual-design}, experience with the relevant programming domain as well as having instructional expertise is necessary in the process of plan identification to accurately identify useful plans suitable for learners. These types of expertise appear to be complementary yet distinct. Attempts to glean programming plans from domain experts alone seem unlikely to be successful without instructional expertise.
%Instructional expertise may be crucial in the attempt to glean programming plans from developers. 
When Arab et al. studied developers' ability to share strategic knowledge, about half of the developers they studied found it difficult to write strategies in a way that novice developers could understand~\cite{Arab_StartegySharingSystem_CHI-2022}.

Simply knowing that a piece of code is common in practice does not solve the problem of plan identification. While this may be a good starting place, instructional and programming expertise is necessary to create a quality programming plan. Those with programming expertise can answer questions about whether the pattern is a meaningful problem-solving step in the domain, and what the goal and intent of the code is. Those with instructional expertise can answer questions about whether the current form of the plan is understandable and usable by students with a particular background. Human expertise is a valuable, and possibly indispensable, part of the plan identification process.

% why instructional
 

% \edit{While }

% % combine both
% \edit{Some participants suggested ways in which educators who understand the concepts of programming plans could work with programmers who understand their programming domain.} 

%\edit{This strategy mimics having the coding expertise to understand the code structure but also prevents being influenced by expert blind spot to keep the plans in favor of the learner's goals.}
% rephrase, this is the language from a quote
% \edit{And that may be a good way to simultaneously have the coding expertise, but not be susceptible to the expert blind spot. }


% this i feel like belongs more in the opportunities section since it deals with the automation
% Such automated metrics may be possible, if the right plan components are available. If programming plans are represented in a format that includes their programming language code, a system could search relevant code repositories for similar code in order to provide a measure of \textit{commonality}. If the system represents programming plans not only in code but also with changeable areas (see Section~\ref{sec:changeable}), then the system can infer how high the level of abstraction based on what percentage of the plan consists of changeable areas, as well as the complexity of typical code in the changeable areas.

% To measure usability, which is the ease with which learners can modify and apply the plan, code comparison with a relevant corpus may not yield much insight. However, it may be possible to get learners involved through a learnersourcing~\cite{weir2015learnersourcing} activity. The system could connect with novice programmers at the appropriate level and give them an automated task to implement the candidate plan. Based on the correctness of this activity, it could provide a metric for usability.





% \subsection{Plan identification in new domains}
% To date, most of the patterns identified have been restricted to a CS1 context. From our interviews, we know about some efforts that are being taken to identify plans in domains other than CS1 including CS0 and advanced level concepts like software testing and data structures. To move towards identifying more patterns in new domains, we investigate about the process that researchers could employ to identify these plans.

% All of our participants believed that to identify patterns in a domain unfamiliar to oneself, one has to first understand the typical structures %find words for this
% or the typical ways of doing things in that domain.
% One of our researchers argued that ,
% \begin{quote}
%     You do things for 'reasons' that you haven't thoroughly examined and that may have negative consequences. (P10)
% \end{quote}
% Thus familiarizing oneself with the domain is a meta requirement. 

%  TEXT THAT NEEDS TO BE MOVED


% \textbf{Ambiguous Plan Definitions: } More than half of our interviewees faced challenges while identifying patterns because of ambiguous plan definitions which lead to uncertainty. 

% P5 revealed that \textit{``There's not really any universal agreement''} in the definition of patterns. This also leads to misunderstanding in the form of different interpretations of any published material. This perplexity has lead to an absence of a \textit{``pattern of finding patterns.''} (P9)

% One of our researchers also confirmed that knowing about the concept of "programming patterns" consciously helped them incorporate this style of instruction for more advanced concepts. \textit{``Now that I sort of know patterns are a thing, I will probably be more aggressively on the lookout for, I'm teaching topics X, Y, and Z. Are any of them amenable to this approach?''} (P7)

==> parking-lot-text/future.tex <==

\edit{\section{Opportunities for Design to Support Programming Plan Identification}}

\begin{figure*}
\centering
\includegraphics[width=\textwidth]{img/design.png}
\caption{A proposed sociotechnical plan identification process that mirrors educators' current plan identification procedures while leveraging both human expertise and automated processing for improved efficiency.}
\label{fig:design}
  \Description{This diagram summarizes the proposed sociotechnical plan identification process. The first box represent the candidate plan identification stage where plans are created based on common code sequences, from literature, or from scratch. There is an arrow that originates from this box to the next box that represents the plan refinement stage showing the successive steps. In the plan refinement stage, we modify the abstraction level of plans and receive automatic and crowd-sourced feedback on metrics. This box has a self-loop arrow representing that it is an iterative process until goal is reached. Then, there is an arrow pointing to a plan library symbolizing that a collection of candidate plans has been created. The last arrow from the plan refinement box is to the last box representing the plan elimination stage. At this stage, if the candidate plan does not reach acceptable metrics or does not meet learning goals, it is discarded.}
\end{figure*}

With a more precise understanding of how plan identification is currently performed by educators, \edit{as well as the barriers in the current process of plan identification,
% as well as an understanding of several opportunities for improving the efficiency of the plan identification process, 
we are able to propose several opportunities for improving educators'} process for plan identification. These new processes mirror the stages of educators' current plan identification procedures, while leveraging both distributed human expertise and automated processing. We describe each \edit{of these avenues} 
% stage of this process 
below and present a summary in Figure~\ref{fig:design}.

% \subsection{Some Plan Structures Better Support Automated Metrics}

% % take a stance
% % We need code in plans to better find the level of abstraction. In plans with just natural language description, it would be difficult to measure the level of abstraction

% \edit{To allow educators and developers to work together, the system must use a consistent plan definition which includes choosing the necessary plan components that best meet the learning goals of the intended audience. We believe that choosing a programming plan definition where plans are defined in code and where plans have changeable areas will best facilitate automated processes that draw on pools of code examples.}

% \subsection{Choice of Plan components and Perspective}

% To allow educators and developers to working together, the system must use a consistent plan definition. Designers of plan identification systems should choose from the list of components (Section~\ref{sec:components}). We believe that choosing a programming plan definition where plans are defined in code and where plans have changeable areas will best facilitate automated processes that draw on pools of code examples.

% Implications for the choice of plan components


%Based on , we believe that a plan definition that uses a solution in code rather than pseudocode or natural language (Section ~\ref{}) presents more opportunities to partially automate the plan identification process because it allows systems to take advantage of the data in existing code repositories, like GitHub or StackOverflow. Further, we believe that the plan representation in a plan identification system should include specific changeable areas (Section~\ref{}), as it enables automatic calculation of the abstraction level . This idea is further explained below in Section~\ref{}.
 
\subsection{\edit{Opportunities to support candidate plan identification}} % Creation stage

% \subsubsection{Opportunity to Involve AI or Data Mining Tools}
% \textit{``Since it learns from so many, it probably has already kind of done the synthesis itself,''} reasoned P6. P6 also suggested that 

\edit{The time-consuming nature of creating a representative, general-purpose programming plan from many examples slows the process of plan identification for educators.}
Reflecting instructors' experiences with plan identification, there are multiple avenues to introduce candidate plans into a system in a way that accelerates the process of plan identification: those that automate the process and those that draw on past work or an educator or programmer's expertise. 

% Some of our educators mentioned that using emerging AI tools like GitHub Co-Pilot (P6) or ChatGPT (P7) to generate solutions could help in plan identification.

First, in order to make the challenging process of plan choice more efficient, a plan identification system can generate candidate plans by searching relevant pools of code for common pieces of code~\cite{haggis_code_similarity}, or by prompting a large language model for examples from a particular domain. Candidate goals and names may also be generated by a large language model. The user can specify the topics they are interested in identifying programming plans for, and the system could then suggest relevant code corpuses drawn from online code repositories (i.e., Github, Stackoverflow) or instructional materials. As educators vary in their beliefs about the type of practice that plans should represent, users should have the ability to limit the code pools used for candidate generation to those by certain types of authors or another measure of quality.

%\edit{Our participants suggested using emerging AI tools to ask for solutions to the same problems in different contexts and then evaluate code similarity to search for plans.}

Another method of candidate plan generation could draw on the instructor's current insight. As some instructors prefer to design their own plans, plan identification systems should include the possibility for users to create a candidate plan from their own intuition. %This process of course depends on a user's programming expertise.

Finally, as some of the educators we interviewed found plans from the literature important in their own plan identification process, systems could allow users to search the existing plan literature as well as programming plans created by other users.

\subsection{\edit{Opportunities to support plan refinement}} %Refinement stage

% \subsubsection{Opportunity for Automated Metrics for Abstraction, Commonality, and Usability}
\edit{We found that plan refinement is an crucial stage in educators' plan identification process, but also an area where educators face challenges as they struggle to find the right balance between a plan's frequency in practice (commonality), ease of use (usability), and appropriateness for their learner population. The process of plan identification could become more efficient if educators could receive quicker and clearer feedback about how their candidate plans measure up in each of these characteristics. }
%evaluating the metrics of plan quality that instructors value could be automated or crowd-sourced.} 

\edit{With automated metrics of commonality,  usability, and level of abstraction, the feedback loop that educators undergo as they search for the right version of their programming plan could be shortened. Such automated metrics may be possible, if the right plan components are available. If programming plans are represented in a format that includes their programming language code, a system could search relevant code repositories for similar code in order to provide a measure of a plan's \textit{commonality}. If the system represents programming plans not only in code but also with changeable areas (see Section~\ref{sec:changeable}), then the system can infer the level of abstraction based on what percentage of the plan consists of changeable areas, as well as the complexity of typical code in the changeable areas.}

\edit{To measure usability, which is the ease with which learners can modify and apply the plan, code comparison with a relevant corpus may not yield much insight. However, it may be possible to get learners involved through a learnersourcing~\cite{weir2015learnersourcing} activity. The system could connect with novice programmers at the appropriate level and give them an automated task to implement the candidate plan. Based on the correctness of this activity, it could provide a metric for usability.}

%\edit{If educators could quickly understand how changes to the programming plan they are refining affect the metrics that they care about, it may increase the efficiency of the plan identification process.}

During the refinement stage of a plan identification system, instructors can edit the candidate plan with the goal of balancing the metrics of commonality, usability, and level of abstraction to values within their desired thresholds. As some instructors value some metrics more than others, users should have the ability to modify the acceptable ranges for each of these metrics. 

As instructors add or remove changeable areas to their plan, they receive feedback from the automated metric values. Instructors' expertise is particularly relevant in the refinement stage, as they not only rely on the system for information about the value of their candidate plan, but also judge its appropriateness themselves. 

\edit{Automated metrics may not completely replace the benefits educators gain from conversations with their peers. In our interviews, we learned that the educators we worked with had extensive conversations about plan identification during their process (see Section~\ref{sec:discussions}). Conversations between educators can also be supported in a plan identification system, perhaps through chats, a commenting system, or suggestions for plan changes.}
%as the instructors we interviewed were clear that these conversations led to improved plan identification outcomes. These reflections on the quality of the plans and conversations can occur through chats and even spontaneous video calls enabled by the system. }

\subsection{\edit{Opportunities to support plan identification in domains unfamiliar to educators}} %Refinement stage

Enabling collaboration between instructors and developers could allow for easier identification of programming plans in specific application areas, as the professional collaborator can suggest plans from their personal expertise or during a guided think-aloud, and the instructor collaborator can refine those plans so they are appropriate for learners. \edit{This approach could make it possible to greatly expand the number of topics where the plan identification process can be applied, as it would no longer depend on a single individual with both types of expertise.}

\edit{Based on our findings, it's important that those with programming expertise and those with instructional expertise contribute in ways that make use of their particular strengths (see Section~\ref{sec:expertise}). For experts in the programming domain, a system could encourage their participation in the candidate plan stage in particular. This may include sharing information about a plan's commonality in a particular domain, as well as information about the intent of a candidate plans. Then, educators may become involved in the plan refinement stage, particularly as they are better positioned to judge how understandable plan components are for the relevant learner level. }

% \subsubsection{Opportunity for Facilitating Discussions Between Educators}


%\subsection{Elimination stage}

%Finally, not all candidate plans will make it into the final plan library. If instructors cannot balance the metrics for a particular plan to acceptable values, or, if the instructors believe that the plan doesn't meet their learning goals, they can remove the plan from consideration. 


==> parking-lot-text/llm-plan-evaluation.tex <==
\section{LLM Plan Generation Evaluation}

To evaluate the plan-ful examples created by generative AI tools, we performed a mixed methods evaluation 
%using quantitative metrics and qualitative analysis based on 
guided by
the characteristics instructors use to judge good programming plans (see Section ~\ref{sec:judging}).
% commonality, usability, and appropriateness for learners.
%to determine the feasibility of using LLMs in programming plan generation.

% Cunningham et al. \cite{Cunningham_PurposeFirstProgramming_CHI-2021} devised a set of programming plans for BeautifulSoup, a Python library, to assist non-majors learn web scraping 

We assessed our programming plans in reference to a set of programming plans identified and used by Cunningham et al. \cite{Cunningham_PurposeFirstProgramming_CHI-2021} to teach web scraping to undergraduate conversational programmers. These plans were designed by researchers with programming plan expertise as well as instructional experience in the domain, and were also validated with web scraping experts~\cite{Cunningham_PurposeFirstProgramming_CHI-2021}. 
To obtain a control set, we extracted the same set of plan components (name, goal, solution, and changeable areas) from the publicly available curriculum\footnote{runestone.academy/ns/books/published/PurposeFirstWebScraping/index.html} and created clusters of plan-ful examples (denoted as \(\mathcal{D}^{\textit{Control}}\)). %in future. 

We also subsampled the generated plan-ful examples in \(\mathcal{D}^{\textit{Plan-ful}}\) to have an equivalent number of examples as the control set. To achieve this, we chose the 10 largest clusters with the most data points and calculated the centroid of each cluster using the embeddings. We then selected the four closest plans to this centroid as the most representative examples in each cluster (compiled together as \(\mathcal{D}^{\textit{Plan-ful*}}\)). 
% Thus, both \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{Plan-ful*}}\) had the same number of examples.

% Our quantitative analysis focuses on analysis of the plan-ful example solutions, in order to understand their validity across the entire datasets and to compare them with non-LLM generated code. Our qualitative analysis was necessary to gain insight about the non-code components of the plan-ful examples, particularly the qualities of goals and plan names.

\subsection{Quantitative Analysis}

\subsubsection{Syntactic Validity}
\label{sec:quant_accuracy}

Before comparing \(\mathcal{D}^{\textit{Plan-ful*}}\) to \(\mathcal{D}^{\textit{Control}}\), we tested the syntactic validity of the generated programs from our original dataset \(\mathcal{D}\).
%, which included 100 complete Python programs. 
We note that from our set of 100 complete Python programs, all but one were syntactically valid. That program included a syntax error and could not be parsed nor executed. Thus, we conclude that the raw code generated by the LLM is mostly accurate and reliable, at least in our target domain. 

% Summary statistics of these errors and their numbers are presented in ~\ref{table:errors}. On closer examination, we find that most of the compilation errors can be accounted to parsing and data cleaning. ChatGPT does not follow a uniform structure while generating its responses. Thus, it was unlikely to ...

%     \begin{table}
%         \caption{Errors in Non-Compiling ChatGPT Code}
%         \centering
%         \label{tab:errors}
%         \begin{tabular}{|p{4.5cm}|p{3cm}|}
%         \toprule
%                 Error Type & Number of Occurences
%         \\\midrule
%             Unterminated String Literal & 8 \\
%             Invalid Syntax & 9 \\
%             Unterminated f-string Literal & 5 \\
%             Unindent Does Not Match Any Outer Indentation Level & 1 \\
            
%         \end{tabular}
%     \end{table}

% This evidence suggests that while there may be some inaccuracies in data generated using generative AI tools, a lot of them can be controlled using a more systematic data cleaning approach.

\subsubsection{Appropriateness for Learners}
\label{sec:quant_learners_appropriateness}

Our instructors emphasized the importance of plans being suitable for their learner audience (Section~\ref{sec:judging}). Thus, we compared \(\mathcal{D}^{\textit{Plan-ful}}\) to \(\mathcal{D}^{\textit{Control}}\) with standard code complexity metrics
%examined the examples in \(\mathcal{D}^{\textit{Plan-ful}}\) in contrast to \(\mathcal{D}^{\textit{Control}}\) using quantitative metrics on four metrics: 
%average lines of code, cyclomatic complexity~\cite{cyclomatic_complexity_mccabe}, Halstead's volume~\cite{halstead_metrics}, and cognitive complexity~\cite{cognitive_complexity_Campbell} 
to determine their suitability for novices: non-comment lines of code, cyclomatic complexity~\cite{cyclomatic_complexity_mccabe}, Halstead volume~\cite{halstead_metrics}, and cognitive complexity~\cite{cognitive_complexity_Campbell}.


%Cyclomatic complexity~\cite{cyclomatic_complexity_mccabe} and cognitive complexity~\cite{cognitive_complexity_Campbell} are measures of the understandability and modification scope of code, whereas
%,  wherein a lower score indicates that the code is easy to understand and modify. We estimate the cyclomatic complexity of each plan and report the mean score in table~\ref{tab:metrics_appropriateness} across each dataset \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{Control}}\). 
%Halstead volume~\cite{halstead_metrics} is representative of the size of a program in terms of its operands and operators and hence also reflective of the code's complexity.
%Analogous to cyclomatic complexity, a lower score is indicative of a more straightforward code snippet. Similar to cyclomatic complexity, the mean Halstead volume score for each dataset in reported in table~\ref{tab:metrics_appropriateness}.
%Cognitive complexity is another metric that estimates the understandability of code proposed by Campbell~\cite{cognitive_complexity_Campbell}.

Table \ref{tab:metrics_appropriateness} shows the mean value for all metrics across the datasets. For all metrics, a lower value indicates a simpler program that is more appropriate for beginning learners. We also conducted a two-sided non-parametric Mann-Whitney U-test for each complexity metric.
%with rank biserial correlation as the effect size. 

While \(\mathcal{D}^{\textit{Control}}\) is marginally less complex compared to generated code according to the metrics, we did not find any statistically significant trends (p $>$ 0.05 for all comparisons). Thus, it is reasonable to claim that the examples generated using ChatGPT can be used in instruction for novices.

% 


\begin{table}
\caption{Mean Code Complexity Metrics}
    \centering
    \label{tab:metrics_appropriateness}
    \begin{tabular}{cccc}
    \toprule
        Metric & \thead{\(\mathcal{D}^{\textit{Plan-ful}}\) \\ (n = 781)} & \thead{\(\mathcal{D}^{\textit{Plan-ful*}}\) \\ (n = 40)} & \thead{\(\mathcal{D}^{\textit{Control}}\) \\ (n = 43)}
    \\\midrule
        % Number of Plan-ful Examples & 781 & 40 & 43 \\
        Lines of Code & 2.30 & 3.10 &  2.72 \\
        Cyclomatic Complexity & 2.43 & 2.21 & 2.40 \\
        Halstead Volume & 173.69 & 178.91 & 114.02 \\
        Cognitive Complexity & 0.217 & 0.375 & 0.233 \\
        % Starsinic Readability & -0.362 & \\
    \end{tabular}
\end{table}

% \[
% \begin{matrix}
%   & \(\mathcal{D}^{\textit{Plan-ful*}}\ & \(\mathcal{D}^{\textit{Plan-ful}}\ \\
%   \(\mathcal{D}^{\textit{Control}}\ & & d 
% \end{matrix}
% \]

\subsubsection{Usability}
\label{sec:quant_usability}

Aside from generating code that is accurate and appropriate for learners, it is also important that programming plans be representative of key functionalities in the domain.
%to provide its users with the flexibility and scaffolding to perform a variety of tasks. 
To this end, we compared the number of distinct method calls used in \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{Control}}\). Having examples on more distinct methods may indicate a set of examples that can be employed to solve a larger number of problems.% (See % (See Figure~\ref{fig:methods-vs-clusters}).

%We found that 
\(\mathcal{D}^{\textit{Control}}\) included four distinct method calls (\texttt{append, find, find\_all, get}), which were also included in \(\mathcal{D}^{\textit{Plan-ful*}}\), the plan-ful examples from the 10 largest clusters generated by the LLM, such as \texttt{select} and \texttt{select\_one}. Moreover, these largest clusters also included five additional methods not included in \(\mathcal{D}^{\textit{Control}}\).
%showing that our clustering algorithm did not cause a loss in method variance. 
This shows that our pipeline generates plans with similar functionality to those designed by an instructor. 



% To examine this behavior more closely, we investigated the number of distinct method calls introduced by each cluster of examples, starting from the largest cluster.
% to illustrate the relationship between the number of distinct methods being used in the clusters as the number of clusters rises. 
% As evident from Figure~\ref{fig:methods-vs-clusters}, 
% By selecting the 10 largest clusters, a majority of distinct methods in the generated set is captured. Moreover, the variance of methods in generated code increases steeply compared to the previously proposed plans.
% almost more of all unique methods present in the set of all generated examples \(\mathcal{D}^{\textit{Plan-ful}}\) are also present in the subset \(\mathcal{D}^{\textit{Plan-ful*}}\). Moreover, 
% follows an upward trend suggesting that more clusters form a larger coverage over the domain's features.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{img/graph-new-pfp-and-gpt.png}
%     \caption{Comparative Analysis of Methods Used As the Number of Clusters Grow in the Plan-ful Examples from ChatGPT}
%     \label{fig:methods-vs-clusters}
% \end{figure}

% We also drew a comparison between the distinct types of methods used in \(\mathcal{D}^{\textit{Control}}\) with \(\mathcal{D}^{\textit{Plan-ful}}\). We find that \(\mathcal{D}^{\textit{Control}}\) encompasses 4 distinct methods including \texttt{['append', 'find', 'find\_all', 'get']} in 6 clusters. The code plans in \(\mathcal{D}^{\textit{Plan-ful}}\) need 7 clusters for addressing these 4 distinct methods. This demonstrates that the ChatGPT generated examples are as varied as the researcher created plans and thus it is unlikely that there will be a loss of variability if examples are generated using AI tools.

% the most common in the D plan-ful have the same methods as D control


\subsubsection{Commonality}
\label{sec:quant_commonality}

A significant motive for using programming plans in instruction is to equip novices with the necessary technical skills to contribute to real-world code problems. Thus, it is essential that plans used in instruction are representative of actual practice.
%to provide learners with the appropriate scaffolding. 
To obtain an estimate of how the LLM-generated plan-ful examples compare to actual practice, we compared \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{Control}}\) to web scraping files from GitHub. We created a new dataset \(\mathcal{D}^{\textit{GitHub}}\) by collecting Python files from public repositories via GitHub's API that met the following criteria: contained a BeautifulSoup import statement, included the BeautifulSoup contructor, and was not a test file. 
%that were written in Python and included the string \textit{BeautifulSoup}
%in any files in any public repository using the publicly available GitHub REST API. This resulted in a collection of 1016 files. We filtered this dataset to include files that had an import statement (\textit{import BeautifulSoup, import bs4, from BeautifulSoup import BeautifulSoup} or \textit{from bs4 import BeautifulSoup} and a constructor initialization (\textit{= BeautifulSoup(}). Finally, we removed test files by filtering any of the following statements: \textit{import unittest, (unittest.TestCase), from bs4.testing import}. 
This resulted in the final dataset with 733 files. Then, we generated the embeddings for these programs using CodeBERT in a similar manner to Section~\ref{sec:clustering} to compare the sets \(\mathcal{D}^{\textit{GitHub}}\) and \(\mathcal{D}^{\textit{Control}}\) as well as \(\mathcal{D}^{\textit{GitHub}}\) and \(\mathcal{D}^{\textit{Plan-ful*}}\).

% To compare the commonality of generated plans \(\mathcal{D}^{\textit{Plan-ful*}}\) to \(\mathcal{D}^{\textit{Control}}\), we compute the distance between embeddings of the code in each dataset to \(\mathcal{D}^{\textit{GitHub}}\). The embeddings for the new datasets are computed with CodeBERT as similar to the prior Section~\ref{sec:clustering}. %, denoted as \(\mathcal{D}^{\textit{GitHub}}\).

%We now compare \(\mathcal{D}^{\textit{Plan-ful}}\), \(\mathcal{D}^{\textit{Control}}\), and \(\mathcal{D}^{\textit{GitHub}}\) where \(\mathcal{D}^{\textit{GitHub}}\) is our baseline, \(\mathcal{D}^{\textit{Plan-ful}}\) is our test set, \(\mathcal{D}^{\textit{Control}}\) is our control set. 
% Using a number of quantitative metrics, we perform analysis that yields information about how the plans compare to real-world code. We first convert the code pieces in \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{GitHub}}\) to embeddings using CodeBERT like before. For \(\mathcal{D}^{\textit{Plan-ful}}\), we use the previously collected embeddings from \(\mathcal{D}^{\textit{Emb}}\). 

% For our first experiment, we compute the average embedding per dataset using a mean of values across each dimension. This yields one multi-dimensional vector per dataset representative of the average embedding of that dataset. Then we perform a cosine distance analysis using functions from the \texttt{sklearn} library in Python on these pairs: \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{GitHub}}\) and \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{GitHub}}\) to gain insight into which dataset is more similar to the baseline. Cosine distance is measured on a scale of 0 to 2 where a value closer to 0 indicates high similarity and a value nearer to 2 represents high dissimilarity. We observe a score of 0.188 between \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{GitHub}}\) and 0.213 between \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{GitHub}}\). Accordingly we infer that the example plans generated using ChatGPT are closer to real-world practice than the purpose-first programming plans. This can be accounted by the fact that LLMs like ChatGPT are trained on public data sources \cite{} whereas the purpose-first programming plans were created by instructors and researchers crafted for novices. We also note the similarity between \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{Control}}\) which is 0.012 which indicates that the LLM generated plans and the purpose-first programming plans are highly similar.

To evaluate the similarity between sets, we computed Hausdorff distance~\cite{tahaEfficientAlgorithmCalculating2015} and Wasserstein distance~\cite{ramdasWassersteinTwoSample2015}, which are common metrics for comparing generated content to reference sets~\cite{pmlr-v70-arjovsky17a, weilihausdorff}. For both Hausdorff (\(\mathcal{D}^{\textit{Plan-ful}}=13.66\), \(\mathcal{D}^{\textit{Control}}=14.92\)) and Wasserstein (\(\mathcal{D}^{\textit{Plan-ful}}=12.97\), \(\mathcal{D}^{\textit{Control}}=13.97\)) distances, the set of generated examples had smaller distance to code from GitHub in comparison to the control set of previously proposed plans, conveying that the ChatGPT can generate plan-ful code that is more representative of real-world examples compared to instructor code.


% We compute Hausdorff distance between sets of embeddings, which is a measure of the maximum distance from a random point in a set to a reference set~\cite{tahaEfficientAlgorithmCalculating2015}. A smaller Hausdorff distance indicates that points for all points in the set have a close corresponding point in the reference set. We found that the distance between \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{GitHub}}\) as 13.66 and the distance between \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{GitHub}}\) as 14.92, suggesting that the ChatGPT generated code pieces are more similar to GitHub examples compared to the plan-ful examples from the purpose-first programming study.

% We also compute the Wasserstein Distance, which is a measure of the similarity of the probability distributions of two sets~\cite{ramdasWassersteinTwoSample2015}. % cost of an optimal transport plan to convert one distribution into the other \cite{}, using in-built functions in the \texttt{scipy} library in Python, between the pairs of the datasets. Analogous to the prior result, 
% Analogous to the previous result, the distance between \(\mathcal{D}^{\textit{Plan-ful}}\) and \(\mathcal{D}^{\textit{GitHub}}\) (12.97) is lesser than the distance between \(\mathcal{D}^{\textit{Control}}\) and \(\mathcal{D}^{\textit{GitHub}}\) (13.97), 
%We also measure the Hausdorff Distance, measure of the discrepancy between two sets of points \cite{}, using the same Python library, among the datasets which also yielded similar results with the score between 

%These findings suggest that examples generated using AI tools are more likely to be used in common code practice, over examples generated by instructors from scratch.

\subsection{Qualitative Evaluation}

To obtain a richer picture of the strengths and weaknesses of plan generation with LLMs, we conducted a qualitative evaluation of the generated plan-ful examples, inspired by thematic analysis approaches in prior work on code generation~\cite{kazemitabaarHowNovicesUse2023}.

We started our analysis with a free-form discussion on both generated plans and previously proposed plans from \(\mathcal{D}^{\textit{Control}}\) to familiarize ourselves with the data. One member of the research team prepared an initial codebook, with codes organized under two main dimensions reflecting the \textit{components} and \textit{characteristics} highlighted in Section \ref{sec:interview_results}.
Two researchers coded a subset of examples (10\% of the data) and obtained inter-rater reliability of 0.76 using percentage agreement\cite{miles1994qualitative}. The codebook was refined through discussion, and two researchers achieved an IRR of 0.89 after the second subset. One member of the team coded the rest of the data according to the refined codebook\footnote{The codebook is available online: https://tinyurl.com/fk6pzat8}.

\subsubsection{Components}
\label{sec:qual_components}

The generated plan-ful examples were `mostly accurate' (90\%, n=36). Only four examples in \(\mathcal{D}^{\textit{Plan-ful*}}\) had `mostly inaccurate' code, indicating that LLMs can generate the solution component of a plan reliably.

Changeable areas of the examples were also somewhat successfully generated: there was only a single case where an unalterable part of the code was annotated as a changeable area. Yet, 22.5\% of examples were missing changeable areas (n=9), and another 22.5\% had changeable areas that were considered `improbable' (n=9). For example, some default arguments of the commonly used functions were annotated as changeable. While technically correct, these areas are not likely to be modified in simpler examples and were not included in previously proposed plans from \(\mathcal{D}^{\textit{Control}}\).

The generation of goals and names was less satisfactory. On the example level, more than half of the generated goals were `descriptive' (55\%, n=22), but 17.5\% of examples were missing a goal label (n=7), and 12.5\% of examples had an `insufficient' or `too general' goal (n=5). On the cluster level, only 40\% of generated names were `descriptive' (n=4), with other names either being `insufficient' to understand when to use a plan (n=2) or `overstating' what the plan actually does (n=4). For example, a cluster that accesses multiple attributes of an object was named ``Data Extraction and Database Management'', even though it does not have any database interaction.

\subsubsection{Characteristics}
\label{sec:qual_characteristics}

The most consistent characteristic in generated examples was commonality: 80\% of examples had `common syntax' with plans placed in the same cluster (n=32) and 67.5\% of them had `common goals' with the plans in the cluster (n=27). Another 12.5\% of examples shared `vague commonalities' (n=5), where it was hard to find the overall goal of the cluster due to great differences in syntax and structure. Moreover, some code statements were repeated in multiple plans (30\%, n=12), and the code for shorter plans, such as importing libraries or calling the BeautifulSoup constructor, was also included within some of the larger plans.

From a usability perspective, most plans were `cohesive' examples of a given use case (67.5\%, n=27), and they were `generalizable' to new contexts (57.5\%, n=23). Moreover, some of the shorter plans did not require customization but could still be useful to students, e.g. ``Importing Libraries''.
% However, some of the other plans were so simple that they would not be beneficial to solve a new problem.
% For example, one of the plans was ``Importing Libraries'' and it just included a set of import statements.

Finally, the appropriateness of the generated content for beginners was questionable: while there were similarities to the ones defined in \(\mathcal{D}^{\textit{Control}}\), 42.5\% of plans used `technical jargon' in the name and goals (n=17). These included revealing some web technologies that were abstracted away in the previously proposed plans, such as GET requests and HTML structure, as seen in Figure \ref{fig:contrasting-cases}. Furthermore, some plans included `advanced concepts' in Python (15\%, n=6) such as list comprehensions or exception handling. 

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{img/contrasting-cases.pdf}
    \caption{Two LLM-generated plan-ful examples from the same cluster, with an example almost identical to an instructor-generated plan from prior work (top), and an example that includes technical jargon and improbable changeable areas, making it potentially confusing for novices (bottom).}
    \label{fig:contrasting-cases}
\end{figure}

% Abstractness


%%%Accuracy

% 36/40 mostly accurate

%%%Quality of Generated Components

%% names
% 4 descriptive
% 2 insufficient
% 4 overstated


%% subgoals
%22 of 40 descriptive
%7 missing
%4 insufficient or 1 too general 

%% changeable areas
%9 missing
%9 improbable
%1 inaccurate

%%%characteristics
% 32 common syntax
% 27 common goal
% 5 vague commonality
% 12 common across

% 27 cohesive and 23 generalizable

% 17 technical jargon
% 6 advanced, 7 confusing


%Appropriateness to Beginners


% \subsection{Results}


%  Accuracy

% A. Are the clusters cohesive?
% B. Are the changeable areas, goal, name, solution accurate?


% Qual


% A. Look at each of the parts
% 	- what do we see



% Quant 

% A. Basic metrics comparison (usability for beginners)
% - lines of code
% - cyclomatic complexity

% B. Embedding distance comparison (commonality)
% - 1. Comparison to GitHub (using prior method)
%     - Which average is closer
%     - How many clusters are closer
%   - # of anomalites

==> parking-lot-text/llm-plan-generation.tex <==
% \begin{figure}
% \centering
% % \includegraphics[width=0.5\textwidth]{img/pipeline-new.png}
% \includegraphics[width=\textwidth]{img/new-plan-pipeline.png}
% \caption{The three stage process for generating example programs, segmenting them with plan components, and clustering these plan-ful examples.
% %collecting and processing responses from ChatGPT into plan-ful examples}
% %\caption{The pipeline for LLM plan generation.}
% }
% \label{fig:llm-methods}
% \end{figure}

\subsubsection{Generating In-Domain Programs}
% Informed by the insights identified in our interview study, we generated programming plans relevant to an application-focused domain: web scraping via BeautifulSoup. We utilized an LLM-based approach to generate these plans with the GPT-4 model from OpenAI using its publicly available API in an iterative workflow. 

Our participants examined example programs and conducted literature reviews (Section \ref{sec:viewing-programs}) as key parts of their plan identification process. Inspired by this, we used Open AI's GPT-4, a state-of-the-art large language model for code generation that is trained on a large corpus of computer programs~\cite{liu2023isyourcode}, to generate candidate programs along with its respective plan components in the programs. First, we prompted the model to generate \texttt{100 use cases of using BeautifulSoup}. Subsequently, we asked the model to \texttt{write pieces of code that use BeautifulSoup to achieve <use case>}. 
% This collection of example programs (which we refer to as 
%dataset 
% $\mathcal{D}$) was used as our primary dataset for further analysis.


\subsubsection{Segmenting Programs Into Plan-ful Examples}
% We then proceed to compile these examples with each of the plan components generated using ChatGPT. We construct a new dataset with these components, Dataset \((\mathcal{D}^{\textit{Comp}})\).
We used the generated programs from
% \mathcal{D}$
the prior step as the input in a set of prompts (see Stage 2 in Figure~\ref{fig:llm-methods}), where each prompt was used to generate one of the plan components identified in our interview study (see Section \ref{sec:components}). 
%We fragmented these generated programs into smaller code pieces by generating \textit{subgoals} in the program. Then, each goal (Section \ref{sec:goal}) and the accompanying code solution (Section \ref{sec:solution}) were added as a single unit of data in our plan-ful example dataset of components, \(\mathcal{D}^{\textit{Plan-ful}}\). For each of these datapoints, we prompted the model to identify \textit{changeable areas} (Section \ref{sec:changeable}). %The name (Section \ref{sec:name}) was determined later in the pipeline (Stage 2 in Figure \ref{fig:llm-methods}).


% From the results of our qualitative study, we now know about the parts of a programming plan. In order to extract these plans automatically, we used ChatGPT. We accessed it using its publicly available API and we used the GPT-4 model. We selected 3 domains that are interesting for non-majors. This included . 

% For each of these domains, we first asked the LLM to generate 100 use cases. We then re-prompted it with the use cases it generated and asked it to generate code that would be written to accomplish that use case.
% potential for another table?
% add code metrics from stackoverflow github work for chatgpt
% With all these code pieces collected, we then asked ChatGPT to generate each of the plan parts one-by-one.

\subsubsection*{Extracting Goals and Solutions}Generated programs 
% in \(\mathcal{D}\) 
typically included a comment before each line, which described that line's functionality. However, these comments did not capture the high-level purpose of the code, as required by a plan goal. To generate more abstract goals for a piece of code, we defined subgoals as \texttt{short descriptions of small pieces of code that do something meaningful} in a prompt and asked the LLM to \texttt{highlight subgoals as comments in the code.} %In our query, we also added the way we define subgoals to provide the relevant context to the model. Specifically, we wrote that 
The output from this prompt was a modified version of each program
% from \(\mathcal{D}\), 
where blocks of code are preceded by a comment describing the goal of that block. % of code. % instead of restating functionality. 

We split each complete program into multiple segments based on these new comments. Thus, the subgoal comments from each complete program I
% n the modified \(\mathcal{D}\) 
became a plan goal, and the code following that comment became the associated solution. %, collected in \(\mathcal{D}^{\textit{Plan-ful}}\). % After it returned the annotated code piece, we extracted the comment and the following lines of code before the next comment. This pair acted as a subgoal-code piece. We collected all such pairs across all use cases from \(\mathcal{D}\) and added them to \(\mathcal{D}^{\textit{Plan-ful}}\).
Each goal 
%(Section \ref{sec:goal}) 
and solution pair
%(Section \ref{sec:solution}) 
was added as a single unit of data in our plan-ful example dataset.
% , \(\mathcal{D}^{\textit{Plan-ful}}\).

\subsubsection*{Extracting Changeable Areas}To annotate the changeable areas for a plan, we defined changeable areas as \texttt{parts of the plan that would change when it is used in a different context} in our prompt and asked the model to \texttt{return the exact part of the code from the line that would change} for all code pieces from the dataset with plan-ful examples.
% from \(\mathcal{D}^{\textit{Plan-ful}}\). 
% This data was added to \(\mathcal{D}^{\textit{Plan-ful}}\).

% to-do
\subsubsection{Clustering Plan-ful Examples into Plans}
\label{sec:clustering}
% We perform k-means clustering on the plans \(\mathcal{D}^{\textit{Plan-ful}}\) to identify clusters of similar code pieces and thus, programming plans.

We used a clustering algorithm to group similar plan-ful examples together as a programming plan. For clustering the code pieces, we used the CodeBERT model from Microsoft \cite{codebert} to obtain embeddings for each code piece in our dataset of plan-ful examples
% in \(\mathcal{D}^{\textit{Plan-ful}}\) 
and applied Principal Component Analysis (PCA) \cite{PCAanalysis} to reduce the dimensionality of the embedding vectors while preserving 90\% of the variance. These embeddings were clustered using the K-means algorithm~\cite{kmeansclustering}. The optimal number of clusters \(\mathcal{K}\) was determined by assessing all possible \(\mathcal{K}\) values 
% (where \(\mathcal{K} \in [2, \texttt{length}(\mathcal{D}^{\textit{Plan-ful}})]\))
using the mean silhouette coefficient \cite{silhouettecoeff}. We assigned each example 
% in \(\mathcal{D}^{\textit{Plan-ful}}\) 
to a cluster of similar code pieces. 

\subsubsection*{Extracting Names}
To generate names for the plan-ful examples, we first defined the properties for a name in the prompt by expressing that \texttt{a name reflects the code's purpose} and it should focus \texttt{what the code is achieving and not the context.} Then, all code snippets from each cluster of examples were provided as input to the LLM along with a prompt asking it to \texttt{devise a name for that cluster of plans}.

==> parking-lot-text/old-interview-study.tex <==
% \section{Interviews of Educational Researchers Who identified programming plans}

%\section{Interviewing Instructors to Unveil The Design Process For Programming Plans}
\section{Understanding the Programming Plan Design Process}
\label{sec:interview_results}
To understand the current process of programming plan identification by educators, we conducted semi-structured interviews with ten computing instructors (see Table~\ref{tab:participants}) who have curated lists of plans for instruction. Mirroring the approach of Fowler et al.~\cite{craig_max_methoda}, we recruited instructors who authored a computing education research publication where plan identification was a part of their methodology or results. Computing education researchers are an ideal source to learn instructional best practices because this population consists largely of instructor-scholars: those who not only teach computing but are also informed by research and recent practices in computing education. This allowed us to discuss their concrete programming plan identification experiences, rather than have participants speculate on the process in general.



% adding sentences to complete the overview

% complete the study overview -- its kinda incomplete
% why those participants and why these methods

%Our literature review showed that authors rarely provide detail about the process they undertake to identify programming plans. To more deeply understand the process of programming plan identification, we interviewed the authors of the publications from the literature review.


% \subsection{Participant selection and recruitment}
% \edit{\subsubsection{Participants}

\begin{table*}
\caption{Participant Demographics.}
    \centering
    \footnotesize
    \label{tab:participants}
    \begin{tabular}{l|ccccccc}
    \toprule
            & \thead{Years in CSEd \\ Research} & \thead{Years in Plans \\ Research} & \thead{Years in CS \\ Instruction} & \thead{Teaches \\ CS1?} & \thead{Uses Plans \\ in Instruction?} & \thead{Industry \\ Experience?}
    \\\midrule
        P1 & 10-20 & 1-3 & 10-20 & Yes  & Yes & Yes \\
        P2 & 5-10 & 4-6 & 10-20 & Yes  & Yes & No \\ 
        P3 & 5-10 & 4-6 & 10-20 & Yes  & Yes & Yes \\ 
        P4 & 1-5 & 1-3 & 5-10 & No  & Yes & Yes \\ 
        P5 & 1-5 & 1-3 & 1-5 & Yes  & Yes & No \\ 
        P6 & 10-20 & 1-3 & 20+ & Yes  & Yes & Yes \\ 
        P7 & 5-10 & 4-6 & 20+ & No  & Yes & Yes \\ 
        P8 & 1-5 & 1-3 & 5-10 & Yes  & Yes & Yes \\ 
        P9 & 20+ & 20+ & 20+ & Yes  & Yes & No \\ 
        P10 & 20+ & 20+ & 20+ & Yes  & Yes & Yes \\ 
    %\\\bottomrule
    \end{tabular}%
\end{table*}

% \edit{\subsubsection{Researcher–Participant Relationship}}
% we were avoiding this

% \subsection{Participant Recruitment}
% \subsubsection{Literature Review of plan identification techniques}

% \subsection{Participant Recruitment}
% To locate individuals who had identified programming plans for educational purposes, we reviewed the computing education and HCI literature for publications where the authors identified programming plans as a part of their methodology or results. We contacted the authors of these papers to request an interview. By targeting the authors of such publications, we were able to ask participants about a specific and concrete programming plan identification progress, rather than have participants speculate on the process in general.



%\edit{Specifically, we tried to identify computing educators who identified novel programming plans in their prior work. While several researchers have designed systems to identify common code sequences , most of such publications just focus on identifying code plans. In this paper, we try to unveil the process and challenges associated with the process of plan identification with a specific focus on their use in pedagogy to meet learner's goals. }


% We searched the ACM digital library within SIGCSE and SIGCHI sponsored venues, as well as the Computer Science Education journal for papers containing any of the following terms:

% \begin{quote}
%    "programming plan*" OR "program plan*" OR "program plan*" OR "programming template*" OR "pattern-oriented instruction" OR "plan-like" OR "unplan-like" 
% \end{quote}

% After eliminating posters and any non-publications, our search resulted in 61 results from SIGCSE sponsored venues, 55 results from SIGCHI sponsored venues, and 5 results from Computer Science Education. 
% The second author reviewed these publications to identify those where the authors specified that they had generated some number of programming plans, and where the programming plans in question were used to understand learners or to design for learners' needs. Papers where the authors explicitly adopted their programming plans from another source were not included. In cases where the second author was unsure about whether the paper met the inclusion criteria, both authors discussed to reach a final conclusion. 
% As the second author reviewed the papers, they used a ``backwards snowball'' process \cite{Claes_SnowballingTechniques_EASE-2014} where works cited by papers in the original search were also included if they met the inclusion criteria. 
% The final set of papers that met the inclusion criteria included 40 publications, dating from 1979-2023. 

% \subsubsection{\edit{Summary of the literature review}}
% \edit{Here we briefly summarize the work of the papers we identified in the literature review.}

% \subsubsection{Selection criteria}
% We contacted the authors of the papers identified in our literature review to request an interview. 
% We began with the first author and moved through the author list until we interviewed an author or all authors were emailed. 
%\edit{We contacted 3-4 educators every week until we reached the end of our duration that we set aside for conducting the interviews and until we reached the end of the shortlisted papers.  We interviewed all educators who showed willingness to answer questions except for any responses we received after the timeline for conducting interviews ended.} 
% We did not contact authors who are no longer active in CSEd research, either because (a) they hadn't published in the last 15 years, or (b) they were a student author who after graduation no longer worked in academia nor published.
%\edit{At the end of each interview, asked participants if they recommended any other potential interviewees.}



% describe why our population is good/why we chose our population

% \subsection{Study Participants}

% Researcher Description
% \edit{\subsubsection{Interviewers:} The first author conducted this study under the active supervision of the second author.  
% % Theyhave been working with the first author since early this year and have a thorough and extensive understanding of the research and its goals. 
% The second author has performed identification of novel programming plans in order to inform the design of curricula.}
% %\edit{In that work, programming plans are influenced by the propositions presented by Soloway.}

% Our ten participants hailed from North America, Europe, and Australasia, with diverse backgrounds that span not only instruction and research, but also industry (see Table~\ref{tab:participants}). Our interviewees included both those early in their teaching careers (1-5 years of instruction experience) as well as those highly senior in their field (20+ years of experience). Most, but not all, taught introductory programming (CS1). Most of our participants had been performing programming plans research for 1-6 years, while a couple had over 20 years of experience. All of our participants used programming plans in their instructional practice.


% better phrase and connect to RQs
% \subsection{Data Collection}
% \subsection{Interviews}
% Our interviews were performed over Zoom, and lasted thirty minutes to one hour. One interviewee requested written communication rather than a Zoom interview. 

% Re-write based on the style of the other paper to include more detail
% \subsection{Study Setup}
We conducted online semi-structured interviews that ranged between 30 minutes and one hour. 
%We noted the extent of their experience teaching and researching with programming plans, as well as their understanding of what a programming plan was. 
%For example, we explicitly asked the interviewees questions related to the time they have spent teaching computer science and researching in computer science education with a particular focus on programming plans research. 
%We also asked questions about their understanding of programming plans in general.
We asked participants to describe the specific activities they undertook to identify programming plans in the paper they authored. This included questions about what they were looking for when they identified programming plans, the resources that were involved in this process, and the procedures they undertook.
We also posed questions to gain insights into the difficulties the interviewees faced when they were identifying programming plans.
%and their ideas of solutions to solve these challenges to identify potential areas where technology can help.}
Lastly, we prompted a discussion about how they would attempt to identify programming plans in a new topic area they were unfamiliar with.
%to move towards automated plan identification in new domains.}

%\edit{During this process, after every section of the questions, we asked follow-up questions for clarifications if necessary.}


% During the interviews, we asked questions about \edit{\textbf{(a) participants' background} to understand the extent of their experience researching with programming plans and its use in instruction, \textbf{(b) their understanding of programming plans generally} to ensure consistency with the definition of a programming plan, \textbf{(c) the specific activities they undertook to identify programming plans in their paper} to deeply understand their process of plan identification, \textbf{(d) challenges they encountered} to identify areas where technology can help, and \textbf{(e) how they would identify programming plans in a new topic area they were unfamiliar with} to move towards automated plan identification in new domains}. 


% \subsection{Qualitative Analysis}
% \subsection{Data Analysis}
We used a transcription service to transcribe the video recordings and used Dedoose, a qualitative analysis software, for coding the transcripts with an inductive, reflexive thematic analysis process \cite{clarke2021thematic}. During coding, we highlighted the connections between the beliefs of our participants and their choices in the pattern identification process. 
Note that while we use the term ``programming plan'' in this paper to clarify our focus on relatively small coding chunks rather than design patterns or architectural patterns, many of the educators we spoke with used ``plan'' and ``pattern'' interchangeably, or even preferred the term ``pattern.''
% Inspired by Causation Coding~\cite{Saldana_CodingManual_2021}, we coded the links between conditions or variables and outcomes.
%, we primarily used Causation Coding~\cite{Saldana_CodingManual_2021}. In this method, codes are designed to highlight the causal beliefs in qualitative data, and include a multi-part structure of outcome, mediating variable, and antecedent condition. 
% For example, one of our codes was ``plans mean different things to different people OR people have different notions of patterns > uncertainty''. 
%This code communicates that the interviewee suggested that people interpret plans differently because of the absence of a definition of a plan. This uncertainty was a part of the challenges they faced while performing plan identification in their study. 
%The phrase before the ``>'' conveys the causal belief or the mediating variable and the phrase after is the outcome.

%refers to inferring ``causal beliefs'' from qualitative data . In Vivo Coding refers to capturing verbatim from the qualitative data to ``honor the participant's voice.'' The preferred coding method was kept as Causation Coding to get to the root of the reasoning behind our participants’ actions to move towards design implications 
% In cases where causation wasn't clear in the transcript, or the participants' own words captured causal information, we applied In Vivo Coding~\cite{Saldana_CodingManual_2021}.
% The first author performed all coding, and both authors met 1-3 times a week over the course of a month to discuss themes among the data.

% \subsection{Reflexivity Statement}

% As our qualitative coding methods are reflexive, we share a statement about the ways in which our experiences may influence our interpretations of the interview data. Similar to our interviewees, we have a history in programming plans research. At the time of the interviews, the first author has performed research with programming plans for eight months, and the second author has performed research about programming plans for five years. The second author also performed a plan identification process as part of their past research, described in [anonymous]. We believe that this personal experience supported us to better understand the processes of the instructors we interviewed. At the same time, we came to this study with our own perspectives about the nature of programming plans, which are most strongly influenced by the work of Soloway and his colleagues~\cite{Soloway1984EmpiricalSO, Soloway_PlansMechanismsExplanations_CACM-1986, soloway_programcomprehensionreview_1988}. 

%% We come from an eliot soloway perspective, so we may be more likely to adpt his ideas. Considered all aspects of transcript. 

% \definecolor{editCol}{RGB}{255,140,0}
% \newcommand{\edit}[1]{{\textcolor{editCol}{#1}}}
%\subsection{Findings from Instructor Interviews}


% Some participants believed...
% In contrast, others thought ....
% Expressed 
% Valued
% Indicated that
% Repeatedly described

%The educators we interviewed described a variety of details about the approaches they utilized and the objectives they hoped to reach during the plan identification process. They also shared challenges and suggestions for potential improvements.



\subsection{Components of Programming Plans} 
\label{sec:components}

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{img/new_plan_comp4.pdf}
 \caption{Components of a programming plan mentioned by our interviewees, illustrated with a common introductory plan.}
\label{fig:plan-components}
  % \Description{This diagram shows the different components of a plan. It has the name of the components along with an example plan with all these components. It has three gray boxes on the top that each depict a part of the plan, including the name of a plan, 
  % this case, Search. The second gray box has 
  % the goal that the plan accomplishes. 
  % For our example, this is to check if the list contains a specific value. The last gray box has 
  % and the rationale behind the plan.
  % % ; in this case, to use the plan to find only one value in the list. 
  % Then, we have three boxes underneath. In our text, we mention that a solution can be presented in the form of a natural language description, pseudo-code or code. Each of these bottom boxes depicts one of these possibilities. The first box has the solution to our example plan in English, the second box to the right has the pseudo code solution, and the last box has the Python solution to our example with the changeable areas highlighted in green.}
\end{figure}

%Our participants had a range of ideas about what a programming plan meant to them.  
% Participants differed in the way they defined a programming plan, as well as which aspects of a programming plan they believed were important to identify.
Our participants looked for a variety of items when they identified programming plans
%In this section, we discuss all plan components mentioned by two or more of the instructors we interviewed 
(see Figure~\ref{fig:plan-components} for a summary). %We include only those components that were mentioned by more than two interviewees.
% More or less specificity about how plans are implemented

\subsubsection{Name}
\label{sec:name}
%For some instructors, programming plans must have a name. 
As P5 put it, \textit{``[plans are] useful common problems that people name.''} The plan name is often reflective of what the plan accomplishes. P6 believed that plans could have \textit{``generic names''} or \textit{``problem-specific names''}, but that the problem-specific names better supported students during problem-solving: \textit{``it was also important for [students] to reflect, `Okay, if I need a counter [plan], what exactly am I counting here?' ''}
The name connects the plan to the types of problems it can solve.

\subsubsection{Goal} 
\label{sec:goal}
%Some of our participants indicated that plans should have goals. This was
A goal, written in natural language, was
a key part of the plan for instructors like P3, who believed \textit{``a plan has to accomplish a specific goal. That was already the starting point.''} 
%However, educators had different perspectives on what a goal meant to them. For some, the goal of the plan is as simple as \textit{``to produce the output that is the solution to the programming problem.''} (P4) %% Commented because KC doesn't understand
For some, a goal emphasizes the deep, underlying structure of certain problem types, even if implementation details differ in practice. This led one instructor to solely focus on goals during plan identification, because
%\begin{quote}
\textit{``according to the programming language you have, the plan can vary. There might be big differences [in syntax], but the goal is the same.''} (P2)
%\end{quote}
%i'm not sure if heart conveys what i'm trying to say, none of the participants actually mentioned this explicitly, for example, we have a stock analyst and they have a list of stocks and they need to find the greatest selling stock, now 'the heart' of the problem in this case would be calculating the max.
% the underlying something?

% subgoal of a problem statement
% underlying structure of the problem
% deep, underlying structure of certain problem types
% Shared outcome of this type of problem
% \subsubsection{Rationale}
% \label{sec:rationale}
% For one of our participants, a programming plan came with a description of the reasons why the plan works and also where it might not. They reasoned that students \textit{``need to look for the reasons behind practice, not just the solutions. This brings insight.''}  (P10)  %\textit{``What are main mistakes that could happen with this one?''} (10)

\subsubsection{Solution}
\label{sec:solution}
For nearly all our participants, a programming plan included some type of solution to the problem it typically solved.
These solutions could be in a variety of forms. Two of our participants thought that implementation in a specific programming language is a key part of a plan. For example, P3 said, \textit{``The code cannot be detached from the way the plan is built.''} P1 agreed, stating \textit{``In order to code in that language in the best way, it's important to understand some of those language-specific patterns.''} 

In contrast, some participants used pseudocode or natural language to describe solutions, in the interest of communicating ideas that would potentially cross languages. In addition to language-specific plans, P1 argued that \textit{``you should be able to explain them abstractly, independent of the syntax of the language''} 
%like, what are you trying to accomplish?''} 
and thus \textit{``in pseudocode you should be able to explain what's going on and talk about what it does and why it gets used.''} However, for P6, writing plans in pseudocode got in the way, and they re-wrote plans in natural language: \textit{``It's really not about the notation...so, for the patterns I went really for just plain English.''}

\subsubsection{Changeable Areas}
% \textbf{Changeable Areas:}
\label{sec:changeable}
Two of our participants used a template-based approach where specific changeable areas in the plan are highlighted. P1 described their approach: \textit{``we use pseudocode, so we with dot, dot, dot on all the [changeable] parts just to highlight, here's the pattern part''}. Similarly, P6 believed that it is crucial to have \textit{``clear instantiation points''} in the solution for the learners while designing plans. %They also felt that the language they used in the plan showed learners where they needed to input specific information:   \textit{``for the English "if", the variable satisfies the conditions, so you know you need to put there a condition.''}. %% Tricky to describe this, commenting out for now

%\textbf{Examples:} One of our participants uses example situations to illustrate the use of the pattern. They do not touch on this aspect in the interview, however, our review of their papers helped us identify this characteristic. 

% \subsubsection{Changeable Areas}


\subsection{Characteristics Used to Judge a Good Programming Plan}
\label{sec:judging}

While different educators had different ideas about what they value in a ``good plan'', we found four themes: commonality, usability, right level of abstraction, and appropriateness for learning goals.
%While some focused on using the patterns effectively giving rise to the ``commonality'' and ``usability'' metrics, others concentrated on pattern design i.e., ``finding the right level of abstraction.'' Thus, we corroborated the following themes about what makes a pattern ``good.''


\subsubsection{Plans Should Be Common}
\label{sec:commonality}
%A spectrum of responses from our interviewees gave us insight into whether it is necessary for a plan to be commonly used in well-written programs.
All but one of the educators we spoke with considered the frequency with which a programming plan is used in practice to be a measure of its worth. As P10 said, \textit{``For it to be a  ``pattern'' it has to be seen in the world. [Plan identification] isn't about creativity, but about exploration and recognition.''}
%These respondents believed that the definition of a programming plan made it \textit{``inevitable''} (P4) that a plan should be frequently employed in standard practice. 
%While our interviewees were generally in agreement that it was important for plans to be used recurrently, 
%However, there were differences in how they judged commonality and how much value they gave to this measure.
% Seeing the programing plan in practice

% Put somehere! Patterns can be based on techniques used in common practice or can be representative of the best practice, two of which may or may not coincide.




%This idea seems trivial for plan identification in an introductory programming context \textit{``Since elementary patterns aren't very  "deep" they are seen in use everywhere.''} (P10) without conscious effort. 

%% This is a great quote but I think it's repetitive
%Yet, sometimes it is also just for patterns to be representative of general implementation approaches used in practice as demonstrated by one of our interviewees, \textit{``But, patterns aren't about "creation" or ["]new ideas". They are about established practice and why it works.''} (P10). 

%P6 suggested a concrete strategy for understanding whether something is common enough to be a programming plan: \textit{``you need to look for at least like three instances in real code to make sure that this is a solution needing a pattern.''}.

% There are different types of common.

% Common to instructional practice
% Common to the world of programmers
% ((((Common enough to solve multiple problems))) Not a real theme??

% But, they had different ideas about the type of practice that was important (instructional practice, and industry practice)

%% Commonality is important, but it's nuanced. There are different types of commonality.

While the instructors we interviewed generally agreed that a good plan should be used frequently in practice, they had different ideas about the \textit{type} of practice that should be used for this measurement. %(instructional practice, and industry practice)
%Throughout the spectrum, we had responses suggesting that commonality is a metric that should be considered during pattern identification, but is not the primary or the deciding factor. 
% One of our interviewees urged caution in what types of programs were used to judge commonality:
% \begin{quote}
%      It's not something where you necessarily want to have a popular vote on things. Just because more people eat at McDonald's than a fancy restaurant doesn't mean that McDonald's is better food. (P1)
% \end{quote}
P1 urged caution in only using general practice to judge commonality:
\textit{``It's not something where you necessarily want to have a popular vote on things. Just because more people eat at McDonald's than a fancy restaurant doesn't mean that McDonald's is better food.''} 

% add the part where the problem itself is usable

Instructors found commonality in instructional resources to be a valid measure of commonality. P1 described two types of commonality, one that draws only from the classroom, and one that draws from professional and other programming practice: \textit{``One is, do we see it a lot in the textbooks and or assignments that we looked at? There's another kind of common, which is when I think about all the programming that happens in the world, is it important in that context also?''} 
%P1 \textit{``And so I think we included things that were common in at least one of those domains.''.} %% Move to process possibly
P6 chose plans based on their frequency in class assignments: \textit{``I was not going to go for patterns if I can't immediately think of at least three or four exercises or questions for the assignments that would need this pattern.''}

%%%% Talk about "usefulness"
% Able to be applied to many contexts? Able to solve many types of problems.
% It must have a clear goal, and I would say that it needs to be useful in many other contexts and ideally have some degree of flexibility to be adapted to similar situations, but it's not always the same, accomplishes a certain goal, but it's useful in many different problems, but flexible enough to be adapted in those different contexts. -P3

% ``frequency of use had merit, but wasn't the overriding concern.'' (p10)
%Only one of our interviewees was not aligned on the value of commonality. They believed that commonality was not crucial, as long as the plan was representative of how a learner thinks (P3). %% Cut for space

% In light of this, our participants also brought to the fore a few resources to validate if plans are common. These include looking at course materials and evaluating the recurrence of patterns, discussing with other people including students, TAs, colleagues, and, using self-introspection to intuit commonality. %% This is more of a process

\subsubsection{Plans Should Be Usable}
\label{sec:usability}
%%% Missing % change as a measure of usability...
Most of our interviewees believed a critical quality of a programming plan is that it can be easily applied to a variety of situations that share similar goals. 
%As P6 described, learners should \textit{``....Easily know how to apply the pattern.''}
P10 said, \textit{``The solution has to be easy to put into practice (with practice).''}
This requires that the plan be adaptable in a way that the learner understands. % while neither needing to be changed entirely nor not needing to be changed at all. 
%its flexibility. To elaborate, it is pivotal for a pattern to be adaptable 
\textit{``Understanding how to tune it should not be the issue''} (P2).

%
% \begin{quote}
%     %It [the pattern] can't be ready to be used for a situation. 
%     You need to adapt [the plan], but you need not to restructure it completely to be used. It should be the right idea to start from. Then you have to fix it for your purpose, to tune it...
%     %, but not just to understand ... 
%     Understanding how to tune it should not be the issue. %(P2) %% Maybe just emphasize this part
% \end{quote}

%The importance instructors placed on usability stemmed from their reasons for teaching with programming plans in the first place. They believed that programming learners often lack the ability to interpret a problem statement and to adapt a similar solution without guidance. As P7 said, \textit{``The bridge between there [the problem] and code is too large.''} %P6 agreed: \textit{``students, of course, always struggled to go from the English description to the code, and so I thought, "Okay, what could we put in between to help them?"} (P6)

A good programming plan supports students to span the gulf between a problem statement and a code solution. P1 described plans as an \textit{``important step between understanding the syntax of a language and understanding how to do problem solving.''} P9 agreed, saying \textit{``knowing the pattern helps getting to a good solution, an expert solution.''} In the same way that interface designers narrow the ``gulf of execution'' between a user's goal and how to achieve that goal~\cite{Norman_UserCenteredSystemDesign_1986}, instructors believed that programming plans should facilitate learners' ability to design and implement solutions.

% Participants motivated the correct level of abstraction by what would help students solve problems. 

%P6 \textit{``I can assure the student has a conceptual understanding before they dive into the weeds''}

%This points us in the direction of finding a bridge between problem solving techniques and their syntactic implementation.
%, which also lays the groundwork behind discussions about whether a pattern should be syntax dependent or language agnostic. 


%A vast majority of our participants believe that the purpose behind a pattern is to push towards conceptual understanding
% another quote if needed
% % So I don't think there's anything magic about patterns. I think it's just, any time that I can assure the student has a conceptual understanding before they dive into the weeds, and then patterns are one way to do that, I guess. 
% and providing \textit{``scaffolding for thinking''} (P6) before diving into syntax implementation. 
% \begin{quote}
%     Before you write a single line of code, let's step back and understand, what's the problem we're trying to solve? And what aspects of that problem are new for you, that you haven't done before? (P7)
% \end{quote}

%% 
% P7 furthered their belief by explaining their process of helping the students learn about the problem conceptually and then start writing code. They thought that they will first present \textit{``examples of the pattern in action''} so that the students don't have to focus on the \textit{``syntax because the scaffolding is there.''} Then, they will \textit{``start pulling the scaffolding away''} so that the students \textit{``begin to learn the syntax.''}

%A usable plan should be easily adaptable by the learner. It should support the learner in translating a problem statement into code.

\subsubsection{Plans Should Have the Right Level of Abstraction} 
\label{sec:abstraction}

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{img/one_col_abstraction_plan.png}
% \caption{An example of more or less abstract versions of the same programming plan.}
% \label{fig:abstraction}
%   % \Description{Three code snippets are shown, with increasingly complex portions of the code snippets marked as changeable areas.}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.5\textwidth]{img/new-balance.png}
% \caption{Relationships between the characteristics educators value when judging quality of programming plans for instruction.}
% \label{fig:metrics}
%   % \Description{A circle in the center for representing the abstraction level. A circle on the top-left for representing commonality. An arrow from the abstraction level to commonality with a plus sign to say that as the abstraction level of a plan increases, it becomes more common and hence establish a positive relationship between these metrics. A circle at the bottom-left expressing usability. An arrow from the abstraction level circle to usability with a negative sign indicating that as abstraction level increases, the plans become less usable. A two-way arrow with a plus sign between commonality and usability to indicate that as usability increases, the plans become more common and vice-versa. Another circle on the center-right for determining the appropriateness of the plan for beginners. An arrow from abstraction level to appropriateness for beginners with a negative sign to say that as plans become more abstract, plans become less appropriate for beginners.}
% \end{figure}

 %Finding just the right level was key to making the plan useful for students.

%Almost all of our participants thought that it is necessary to find the right level of abstraction for designing patterns. 
%Finding the right balance between concrete and general was key for most of our interviewees when identifying programming plans. 
Pinpointing the right level of abstraction or \textit{``granularity''} (P3) in a plan should ensure that the plan can be applied across multiple contexts, while also providing sufficient concrete detail to support learners to implement the plan in practice. 
% Figure~\ref{fig:abstraction} shows how changing the parts of a plan can lead to more or less abstraction.

% \begin{quote}
%     If you list too many [plans], you lose the idea of the schema, the schemata to it. If it is too abstract, you cannot use it in practice. Students have difficulties in grasping the idea and using them. (P2)
% \end{quote} 

% This is about experience level.
% Furthermore, P6 underlined,
% \begin{quote}
%     ...  
%     %  experiencing in program, that's
%     when we are more experienced in programming, that's also the way we think. ... we are looking at the problem already at the more abstract level." So it was also to convey and to make explicit the kinds of things that probably go on in our minds, but often they are not verbalized or declared. (P6)
% \end{quote}

% What does abstraction mean in terms of programming plans? Instructors defined this concept in terms of how much change students had to implent to put a plan into action.

% Not unchanged, but not totally changable. 
P2 cautioned that plans must be applicable in multiple contexts, saying \textit{``If it is too specific, it's not recurrent enough.''} and students might see the plan \textit{``as a recipe expected to be ready to be used.''} On the other hand, P2 believed it is essential to ensure the plan is not \textit{``too abstract''} so that students \textit{``have difficulties in grasping the idea and using [the plans].''}

% This could be because the instructors want learners to gain expertise, which they see as having genreral schemas. More expertise == more abstract schemas! \cite{}

The educators we interviewed believed that the right level of abstraction was impacted by the intended audience for the programming plan. 
%One of the other researchers also highlighted the importance of \textit{``teaching by diminishing deception''} (P1). They 
Most participants thought it is essential to \textit{``teach novices and experts patterns very differently''} (P1). This is because \textit{``advanced students can handle more abstract explanations''} (P10). 

%P1 believed that as students gather more expertise, it could be useful to then introduce \textit{``more advanced defined patterns''} and emphasize \textit{``the wrong ways to do things and why this solution is better''}. By contrast, a good plan for beginners is relatively \textit{``concrete''}, and focuses on \textit{``how you solve this problem''}. P3 shared that \textit{``it doesn't make sense to talk about plans in general''} since for \textit{``high school students, even declaring a variable is a plan and later they move on to complex plans''}.

%This goal and presentation disparity in patterns for advanced students and novices may or may not overlap with each other. For example, P3 said that \textit{``with high school students''} or novices, they \textit{``don't show them the inner parts''} and focus on the \textit{``goals''} over \textit{``details''}. They start introducing these goals in \textit{``undergraduate courses''}. They also highlighted that 


% Some participants described good plans for beginners as different than plans that were best for experts. These researchers believed that a good plan for novices is relatively ``concrete'' (PX). PX shared, 
% \textit{``Yeah, again, so the abstract thing is talking about... A lot of times patterns are in the design patterns book for example, they're introduced using UML diagrams, whereas }


% PX shared, ``we use pseudocode and actual pieces of code...it is just a much more concrete representation versus something like UML %end here?

% , which is...
% %just like, we blow these kids away and it's [UML is] 
% useful for more sophisticated things than we're introducing.'' 
% 3

% PX believed that as students gather more expertise, it could be useful to then introduce the ``properties of the solution.''

% And then we don't sort of say... I think in more advanced defined patterns, you might talk about thing the wrong ways to do things and why this solution is better, sort of the properties of the solution. Whereas we would just say, "This is how you solve this problem.''




% difference in goal
% difference in content
% difference in presentation influenced by prior knowledge
% i think that's all the kinds of differences i saw

% Following these claims, it becomes necessary to understand whether the design of patterns should be different for learners with different levels of expertise. This raises the question if patterns different 
% % trying to write something like 'in terms of content' -- like idk maybe for loops for summing for beginners and connecting to an api for more advanced students
% % unsure of how to phrase it correctly
% % in terms of content?? -- contentually
% conceptually and content-ually for people with different levels of expertise or is the difference only at the presentation level. 





 

% \subsubsection{Plans Should Meet Learning Goals}
\subsubsection{Plans Should Be Appropriate for Learning Goals}% of Students}
\label{sec:learning-goals}
%% The content varies by novice vs expert, and the level of abstraction varies between novice vs expert.

One of our interviewees highlighted that from a \textit{``teaching perspective''} (P8), a quality plan should be appropriate to the learners' goals. They elaborated, \textit{``if you're in the beginner level, you definitely want to understand what is a programming language, how do I do stuff?''} For those learners, better plans illustrated the operation of language features, to \textit{``help [them] build an idea of [their] notional machine''}~\cite{sorva_notional_2013}. However, for more advanced students, \textit{``you probably want to prepare for industry,''} so ideal plans would be representative of the \textit{``most recent programming paradigms''} (P8). 

%P5 exemplified that \textit{``there are patterns for system architecture and if we're lecture one of CS101 and said, "All right here are some system architecture patterns," I think that would maybe not help too much.''} %% Not my fave quote KC

%Most of our participants believed that due to the differences in prior knowledge and familiarity with different types of content, the \textit{``content that they [learners] would learn would be different for more novice versus more advanced learners''} (P8).

% \begin{quote}
%     So you would "probably, a program plan that is more based on those paradigms would be much more useful for me. Still, the other one could be good from a teaching perspective because it tells me so many things about how program language works, how the computer works, it helps me build an idea of my notional machine.(P8)
% \end{quote}

%if you're in the beginner level, you definitely want to understand what is a programming language, how do I do stuff? And later, you probably want to prepare for industry, so you want to definitely know about those things so this is definitely a difference in goal. (P8)

% difference in presentation



% For example, sometimes with the high school students, I just say like, "Yep, the goal is to be able to repeat something." They don't need to know the details. The plan that I'm presenting to them is a repetition of X steps. I don't show them the inner parts, the inner sub plans that are there. That's something that I usually actually do on the undergraduate courses. 

% It doesn't make sense to talk about plans in general. For my high school students, beginners, plans for them, declaring of creating a variable, it's a plan for them. Maybe the beginning, later they move on to more complex plans and so on. (P3)


%% include in final?
% Thus, for these participants, an ideal plan is independent of programming languages and helps a student focus on the structure of the solution before getting into its mechanics. 
% Some other reasons supporting this argument include flexibility and freedom of using language independent plans and the need for being able to solve problems across languages using the same patterns. 

% However, two (P1, P3) of our participants believed that a pattern should in fact be language dependent as highlighted in the previous section.




\subsection{The Process of Plan Identification}
\label{sec:process_intro_plan_design}
Our interviewees took diverse approaches to identify programming plans. While some educators focused on techniques that helped them gather insight from common practice,
%(such as ``looking at sample programs'', ``having discussions'',  or``doing a literature review'') 
others relied on their personal expertise. Most of the educators we interviewed leveraged a combination of both these strategies. 

% The following subsections detail each activity educators undertook to identify programming plans.

\subsubsection{Viewing Programs and Problems}
\label{sec:viewing-programs}
Echoing the belief that \textit{``patterns are "mined" from the practice''} (P10), many educators looked at some sort of code, problem statement, or instructional material during their plan identification process. More specifically, they looked at GitHub repositories (P7), programs written by industry professionals which may or may not include their own code (P7, P8, P10), textbooks (P1, P2, P5), and other instructional material including lecture notes, assignments, student programs, and testing material (P1, P2, P4, P6, P9).

\begin{quote}
``There was a lot of just paging through textbooks, either physical or digital versions and just looking at code, just trying to see if there's something we haven't seen before.'' (P1)
\end{quote}

% During this approach, we could say that the patterns that are thus created are largely influenced by others' designs including \textit{``language designers, pattern related content publishers''} (P5), instructors, and so forth. 
% One of our interviewees emphasized this idea by claiming that,
% \begin{quote}
%     Patterns are discovered in practice, not invented. Patterns are "mined" from the practice. (P10)
% \end{quote}

As the educators reviewed this content, their own expertise and experience played a role in finding the programming plans. \textit{``You know it when you see it,''}  said P7. P10 highlighted that gathering plans from common practice is not independent of the identifier's own perspective: \textit{``there's a personal selection path that always happens.''} 
%During the review of the sample programs, problems, and instructional content, the educators used their past experiences as instructors, programmers, or both. Some researchers stressed on this fact by claiming that  Another approach is to identify recurrent pieces of code and then use personal expertise to determine if they are worthy of being "patterns." 

% In addition, another one of our participants highlighted that even when the researchers use intuition to come up with patterns, it is another instance of identifying patterns based on others' designs since their experience is also influenced by what is common practice. 
% \begin{quote}
%     ...we're already impacted, affected by what we've seen. (P2)
% \end{quote}  



\subsubsection{Creating Initial Candidates}
\label{sec:process-candidates}
% \subsubsection{Discussions}
% \label{sec:discussions}

We observed that most of our interviewees followed an iterative approach, starting with initial candidate plans and refining them through various approaches. 

Collaboration was highlighted to be helpful for the plan identification process. \textit{``The teamwork was very helpful,''}  said P9. Collaboration could involve discussions with co-authors (P1, P2, P3, P7, P9, P10), co-instructors (P8, P9), TAs (P4, P8), paper reviewers (P5), study participants (P4), other researchers (P7, P9), and developers in the industry (P8). 
 %One of the interviewees reasoned that individual perspectives alone cannot be considered representative of common practice because they thought that it is \textit{``very likely their experience is different from another person's experience.''} (P8) 
% the following line can maybe be shortened and summarized
%They added that discussions with \textit{``people from different levels, different cultures, different student beginners levels, advanced student, people in industry, people in different countries. People who maybe came from a totally different background, they didn't want to learn programming to be a programmer, but maybe to just analyze data, became data scientists.''} (P8) to consider different perspectives is crucial in the pattern identification process.
These discussions occurred across different stages of the plan identification process including from when candidate plans are first presented, to when they are refined into their final form or removed from consideration. 
% Below we summarize the types of discussions that occurred over time, 


% \textbf{Identification Discussions}: 
While identifying patterns, P9 highlighted that they talked about most of the components of the plan including \textit{``what to name a pattern''}, 
%\textit{``choosing problems''}, 
\textit{``how to write this pseudocode so it can be generalized to different languages''}, and the difference between language constructs and plans, i.e., \textit{``maybe this is not a plan, it's just an idea how to do it right.''}
P1 highlighted that they deliberated about which plans to include in their final inventory: \textit{``we just talked about them, be like, ``Yeah, that's really kind of arcane. Maybe that's not a general purpose pattern.''} or {\textit{``Oh yeah, that makes a lot of sense.''}} 

% P3 endorsed this assertion by detailing the role of discussions in their plan identification process by saying, \textit{``Yes, a lot with [co-author] and we discussed it a lot, particularly the level of granularity that we should aim for. We didn't know if we should add the very small stuff, like memory, location and so on.''}

% \textbf{Refinement Discussions}: 
% Some of the researchers created an inventory of patterns and then used discussions to refine their patterns. For example, one of our participants created a set of candidate plans based on their personal preferences and then conducted discussions with other contributors to deliberate on the plan properties and whether the plan was good enough to include in their final list. 

% \begin{quote}
%     This was done, I should say iteratively. We're starting with something, we discussed, we found something that could be reasonable, and we start analyzing some real materials, real instructors material and check if something was left out, wasn't covered or wasn't recurrent enough. (P2)
% \end{quote}

% the following para can maybe be put across some other way
% One of our participants decided to take an indirect approach in this refinement stage where they did not discuss the constituents of the plan directly but asked their co-authors and TAs about \textit{``How complex does [the plan] feel to [them]?''} (P8) and then they redefined their patterns according to the responses to the question. This is because they believe that \textit{``complexity is a proxy for how much do I know it?''} To elaborate, they suppose that \textit{``If I know something, no matter how complex it is, I think it's simple. If I don't know it, even if it's a little bit simple, I would think it's still complex.''}

% \textbf{Decision Discussions: } 
%P1 highlighted that they deliberated about which plans to include in their final inventory: \textit{``we just talked about them, be like, ``Yeah, that's really kind of arcane. Maybe that's not a general purpose pattern.''} or {``Oh yeah, that makes a lot of sense.''} 
%P10 explained that their plan identification process included \textit{``discussions about the ``why" and ``why not".''} %% Maybe this is about rationale? KC

% \subsubsection{Literature Review}
% \label{sec:lit-review}
As another approach for creating candidates, almost all of our participants conducted a literature review to take inspiration from the existing patterns and tailor it to their vision. \textit{``Having a bunch of literature of course helps a lot,'}' shared P8. \textit{``We also took those [plans from literature] because they were broadly researched, people talked about it, so we had some benchmarks.''} But finding a plan in the literature wasn't always the end of the search. P8 shared that they don't take plans from the literature as the final word.
\begin{quote}
Someone telling you this is a good candidate for a programming plan, you still have to think, is it still a programming plan? Or maybe not. Is it only for this particular context? (P8)
\end{quote}

\subsubsection{Finalizing Plan Design}
\label{sec:individual-design}

The final step in this process was refining the candidate plans into programming plans appropriate for teaching.
All of our interviewees have teaching experience, and most of them have had long careers as instructors (see Table \ref{tab:participants}). Instructional expertise is helpful for transmitting programming plans effectively to an audience of learners. As \textit{``plans are useful only if they can be communicated between humans''} (P1), it's important for plans to be appropriate for the knowledge level of the audience. One of our interviewees also highlighted that a plan identifier needs to have relevant programming background or find it in someone else: \textit{``...you need some experience in that practice or the ability to have discussions with people who have that experience''} (P10).
These instructors believed that only those with expertise in a programming topic could shed light on the crucial issue of code's intent. As P4 described such knowledge: \textit{``
%Is this a pattern or is this just a construct of your language? 
Is this an unfortunate oddity of syntax, or is this actually something that means something to you in your domain?''}

Thus, one of the techniques employed by our interviewees was to draw on their experience in order to come up with plans on their own. By considering important problems and exploring \textit{``how you would imagine best solving the problem''} (P9), the instructors generated first draft programming plans they could refine and use in instruction. Envisioning assignments at the appropriate level and inferring relevant plans was a similar strategy for some: \textit{``just also thinking about what's an interesting ten line program that you can assign students to write.''} (P1) \textit{``Now what other simple problem do I want?...Okay, let's try to encapsulate that as a pattern''} (P6)

% Just putting this other quote here in case can be used
% "Now what other simple problem do I want? A simple type of problem, do I want them to be able to solve?" And so then, "Okay, let's try to encapsulate that as a pattern."

With this strategy, the instructors used their own expertise to complement searching through the literature or example programs: \textit{``I knew that's the way you solved the problem so, in a way, I didn't need any kind of evidence.''} (P6)

%% Commented out as too distant from the theme
% People who identified patterns in a CS1 context, argued that sometimes their patterns might seem quite similar to others' even after self-identification since there aren't too many new ways to achieve the same goal. For example, 

% \begin{quote}
%     ... but in essence [the plan] seemed to be the same. Because, as I said, there are not many ways of iterating over a list or counting or summing things up. (P6)
% \end{quote}

% Some other tools that researchers used to identify patterns included looking at the \textit{``higher order functions''} (P5) existing in high-level languages since they are representative of common goals in programming. Sometimes, the way of identifying patterns for some researchers was also influenced by the flow of content in their instruction as illustrated by P6, \textit{``and the problems were chosen based on prior assignments''}.

% In light of this, our participants also brought to the fore that these resources can also be used to validate if plans are common. 
% These include looking at course materials and evaluating the recurrence of patterns, discussing with other people including students, TAs, colleagues, and, using self-introspection to intuit commonality.
% All of these approaches help researchers create an inventory of candidate plans.

% \subsection{How Expertise Influences the Plan Identification Process}
% \label{sec:expertise}
% Many of our interviewees could reflect on long careers that included both instruction and industry experience (see Table~\ref{tab:participants}). As P10 put it, their team of plan identifiers had \textit{``long experience both with programming and with teaching it.''} From our interviews, it was clear that our participants drew on two distinct types of expertise as they identified programming plans: their  \textit{instructional expertise} and their \textit{programming expertise}. We found that these types of expertise are distinct but complementary. 

% \subsubsection{Instructor expertise supports judgment of a plan's appropriateness for learners}
% \label{sec:instructor-expertise}
% Instructional expertise helps the plan identifier with aspects of plan identification related to transmitting programming plans effectively to an audience of learners. As \textit{``plans are useful only if they can be communicated between humans''} (P1), it's important for plans to be appropriate for the knowledge level of the audience. Fortunately, instructional expertise made our plan identifiers ready for the job: \textit{``This is one of the things that academics do, we reinterpret things in terms that are easier to teach to people''}~(P7).

% The instructors believed that their teaching experience gave them insight into \textit{``....the mental state of the person that's going to receive this information and how do I communicate that effectively?''} (P1). During the plan identification process, our educators put themselves in the minds of their students. P3 described this process: \textit{``we imagine, this is what students would have to learn from scratch. This is day one.''} This understanding helps them in refining plans so they are an appropriate bridge for problem-solving. P3 described this as a  \textit{``process that takes a lot of time and a very deep understanding on what you're trying to accomplish and who is your audience that you are trying to create those plans.''} 


% EXPERTISE: Instructors seem to have a sense for what the right usability level is for their students.

% About applying the plan model
%``We always have these very lengthy discussions on what is a plan for you? What is a plan for your students and what is your notional machine? Yeah, that's a ''

% The process is lengthly, and requires a large amount of instructor expertise about what your learning goals are and what your audience understands.

%In another scenario, while having discussion with programmers, this teaching experience can help get rid of \textit{``expert blind spot.''} (P8)

%Both experiences give the pattern identifiers the skill set for self-examination of patterns which helps create a set of candidate plans. 
% Area is important. Where do I mention this?

% \subsubsection{Programming expertise supports judgment of a plan's frequency in practice} 
% \label{sec:programmer-expertise}
% Programming experience also played a role in understanding the value of candidate programming plans. % \subsubsection{Opportunity to Foster Collaboration between Educators and Developers}
% As P7 described, \textit{``In my case, I had a large internal vocabulary of examples already because of my own mileage in code writing.''} P8 agreed that programming experience \textit{``gives you a huge pool of examples.''}

% Not only does programming experience give a plan identifier a set of sample plans, it also equips them to reflect on their own code writing process to inform the plan identification process. P7 highlighted that one can \textit{``think back''} to consider what part of their code writing process was \textit{``easy or hard''}. They also added that during this process, it is possible to find \textit{``sets of features that separate different categories''} of plans.

% One of our participants mentioned that an advantage of having this experience was how it supported them to make judgments about candidate plans:
% \textit{``If you don't know it [the candidate plan] and you already saw so much, I think it's very unlikely that someone else knows.''} (P8)
% Without this expertise, a plan identifier would have to have more discussions with people with this expertise which is a time-consuming process.

% One of our interviewees also highlighted that a plan identifier needs to have relevant programming background or find it in someone else: \textit{``...you need some experience in that practice or the ability to have discussions with people who have that experience''} (P10).
% These instructors believed that only those with expertise in a programming topic could shed light on the crucial issue of code's intent. As P4 described such knowledge: \textit{``Is this a pattern or is this just a construct of your language? Is this an unfortunate oddity of syntax, or is this actually something that means something to you in your domain?''}

%In addition, one also gets access to a large dataset of code for identifying patterns in the form of code written in the past of lecture notes. P7 endorsed this claim by saying, 
% to think about the challenges that they faced while writing code. They could also think about the times where they had to achieve the same goal in different contexts and then evaluate the similarities and differences in the code that they wrote.
% quote -- So if I sort of start to think back and say, all right, what made these test cases easy, hard, whatever? Is there a set of features that separate this category from that category of tests?

% This could help identify patterns since finding the "pattern" is at the core of the pattern identification process.

%``I went for a...software development internship. And also there, I saw people using those plans and also talking about code using those plans. So they were not saying, and here's a for loop and here's a variable...they said to us, "And here we compute a maximum, here we have minimum, here we have the sum, here we have the average".'' (P8)


% look at what others who are working or doing stuff in this domain

% \subsubsection{Something}
% % hmm it doesnt color the subsubsection headings, maybe we don't even need one
% but without it, it seems to be a part of programming
% \label{sec:something}

% \edit{Some participants suggested ways in which educators who understand the concepts of programming plans could work with programmers who understand their programming domain:
% \begin{quote}
% %I think one thing that we didn't do, which I think could be interesting, again, 
% ...if you're trying to find novel patterns...
% %, would be to 
% sit down with a developer at a real company and just have them walk you through the code and explain what's going on. And that may be a good way to simultaneously have the coding expertise, but not be susceptible to the expert blind spot. 
% % %Because if you have somebody who doesn't understand the code and the person's explaining it to you, you sort of get both of those things that they have to be explicit about why they're doing the things that they're doing 
% (P1)
% \end{quote}}

% %One of our participants said that one could work with a \textit{``forwards''} (P4) approach to consider expert opinions while identifying plans where one asks the expert about things that \textit{``mean something''} to them. Or, one could take a \textit{``backwards''} approach and create a set of candidate plans and then ask the expert if those patterns are important. 


\subsection{Challenges}
\label{sec:challenges}

While our participants had all successfully identified programming plans to be used in an educational context, they did name some challenges they experienced in their process, or imagined challenges for future plan identification. % These cOur participants expressed that they faced challenges while identifying plans from practice and while choosing the suitable level of abstraction of these plans for their audience.}

%Identifying the predicaments in the plan identification process will help us get closer to uncovering design implications. Thus, this section highlights the challenges that our participants faced while identifying patterns.

\subsubsection{The Challenge of Choosing Plans from Practice (C1)} 
\label{sec:challenges_practice}
While our participants had ready access to resources that could be used to identify plans, like example programs and problems, they still found it onerous to translate this practice into plans. As P7 described, \textit{``the challenge was trying to infer general characteristics from a large collection of specific examples.''} Another participant described this part of the process as \textit{``tedious''} (P1). 
% \edit{One of our participants expressed that they faced uncertainty while \textit{``defining the plan''} because they had \textit{``ambiguous definitions (P2).''}}

This challenge is particularly relevant when educators ``mine'' plans from existing materials, a technique that the vast majority of our participants employed during plan identification (see Section \ref{sec:viewing-programs}). Understandably, determining which aspects of a given example are widely applicable enough to ``count'' as a programming plan is a difficult task, as the possibilities for writing programs are so extensive. Currently, plan identifiers lean on a combination of their own expertise and a manual search of examples as they tackle this challenge.
% Our plan identifiers this search space can be quite large, leading to a lengthy exploration for something that qualifies as a common pattern.  
%We found that it is difficult for educators to identify programming plans from practice because the search space can be quite large. %When instructors lack the programming expertise to evaluate the meaningfulness of potential plans, it also becomes highly challenging to identify plans.

\subsubsection{The Challenge of Finding the Right Abstraction Level for a Plan (C2)} 
\label{sec:challenges_abstraction}
Once plans are chosen, the challenge only begins. As mentioned previously, finding the right amount of abstraction is key in identifying good plans, according to computing educators. However, finding the appropriate balance of specific and general was a hurdle in our interviewees' plan identification process. 

\begin{quote}
    The difficult part is probably defin[ing] the level. What's the plan you are looking for, how general it is. Level of generality, abstraction to define it. (P2)
\end{quote}

P7 illustrated their challenge by describing the conflicting goals of this process: a good plan should be \textit{far enough above the level of code that it really does insulate students from syntax and mechanics, but not so far that it becomes useless.} Currently, educators make use of discussions with colleagues as one approach to manage this difficulty. On an even longer time frame, they may also refine their plans after seeing how they work in the classroom.

% \begin{quote}
%     But trying to infer what the pattern would be that they had in common was the hard part. (P7)
% \end{quote}

%% This challenge doesn't come across as convincing to me
% \subsubsection{Designing Patterns}
% Even though some of our interviewees believed that defining patterns is not as hard as identifying patterns, \textit{``I don't think we have problems defining them, maybe choosing them.''} (P9), there were some considerable challenges while designing patterns that came across in the transcripts. Most of these challenges were associated with putting the identified patterns in the form of a structure that meets the definition of a "pattern and
% that best fit their audience like \textit{``Maybe I should rephrase this a little bit so that it becomes more consistent across the patterns.''} (P6)

%% Not super convincing and the talking with students is maybe not the best example. But maybe I'll change it back.
% \subsubsection{Communication and Collaboration Barriers}
% One of our participants encountered impediments in the form of language barriers while conducting their plan identification study because it involved oral exchanges. P4 highlighted that gathering intent from students about their planning process, although better than just interpreting code, still comes with its hardships. For example, \textit{``"they just didn't know what they were doing and throwing whatever at the wall, see what sticks"''} and \textit{``"some students English wasn't as clear as others, whether it's because they were trying to do it shorthand, whether it's because we have students who English isn't their first language."''}

% Moreover, some of our participants emphasized the importance of collaboration in the pattern identification process, for example, \textit{``Most of the work in programming patterns was highly collaborative. A group of us would meet once or twice a year for several days and kick ideas about.''} (P10). One of our participants, thus highlighted distance as a struggle however, we believe that the new technological advancements would help reduce such hardships. 


\subsubsection{The Challenge of Identifying Plans in an Unfamiliar Domain (C3)}
Identifying programming plans from more programming topic areas beyond introductory programming could enable better support of learners with diverse interests. However, when we asked our participants about how they would identify programming plans in a new and unfamiliar domain, nearly every one said that it would be quite challenging. Our educators were quick to emphasize the importance of having programming expertise in the relevant topic when performing plan identification.  \textit{``Looking for material and try to recognize the schema without having expertise in the area, I think that would be impossible,''} said P2.

The key hurdle our participants anticipated in identifying plans from new domains was not finding common code, but understanding if that code implemented a meaningful goal. The task of identifying plans for educational purposes is multifaceted: it involves understanding \textit{``what goals [students] need to achieve in this particular context''} and \textit{``how much do they know at this point in their instruction''} (P3). While educators might understand what students are ready to learn, they cannot understand the important subgoals and tasks of a programming domain without the relevant expertise.

Several participants suggested collaborating with an expert from the relevant domain to understand the \textit{``typical things [experts] need to do and how [those are] typically done} (P2). This discussion was necessary to \textit{``discover the intent behind code''} (P1), which is challenging to discover from looking at code alone. Some of our educators mentioned that using emerging AI tools like GitHub Co-Pilot (P6) or ChatGPT (P7) to generate solutions may also help with plan identification when plan identifiers lacked the relevant expertise.

%``why they're doing what they're doing'' (P1), Need to ask a domain expert ``does this actually mean something to you?'' (P4)

% more quotes for this section

% P1
% somebody to sit down with you and walk you through, pick up a representative piece of software for doing that, explaining why they're doing what they're doing
% I think the intent is one of the things that's often hardest to discover in large pieces of code and that people may be much better at explaining what the code is doing rather than why it's doing. 
% And I think a virtue of pattern is that it should hopefully represent best practice or at least good practice.

% P2
% I'd find an expert and ask them what are typical things you need to do and show me how this is typically done. 

% P3
% Well, then I would first have to understand what are the constituents of this context, so what students need to perform and what goals they need to achieve in this particular context. 
% hen I would look into how much do they know at this point in their instruction and match those and say, "Oh, this is enough."
% What kind of actions do they have available? What are the rule sets? What are the goals they need to achieve?

% P5
% I don't know if there are textbooks on web scraping, but looking at some kind of rigorous sources on web scraping, seeing what do people do? How do they describe these things? Are there threads of commonality between different resources?

% P4
% And so that there's sort of the backwards and forwards being able to do that program analysis and then go to a domain expert and be like, does this actually mean something to you? And then going to the domain expert and be like, okay, what means something to you? What are the patterns that you're commonly using? And then can you show me? 

% Some of our educators mentioned that using emerging AI tools like GitHub Co-Pilot (P6) or ChatGPT (P7) to generate solutions could help in plan identification.

% P8
% I would probably look at what others who are working or doing stuff in this domain, how would they do things and how would they solve common problems? What are common problems, what are common solutions to that problems?
% And then they started explaining what features they like to have in there and it helped me a lot to see how they argue about things, because they started arguing about things on a very different level than I expect because they have different ways of thinking about things.

% % addressing the third challenge
%\edit{While conducting the study, we presented our interviewees with a hypothetical scenario in which they had to identify plans in a domain that they were not knowledgeable about. We asked them about how the process of plan identification would be similar or different in that scenario. While our interviewees did not perform plan identification in domains unfamiliar to them, they suggested that collaboration with experts from those particular domains could yield insights into the code's intent (Section 4.4.2). With these conversations, then these instructors would be able to use their educational expertise to create plans from those domains.}

==> parking-lot-text/parking-lot.tex <==
\subsection{Solutions-first vs problems-first}
% Our participants varied in the way they defined a programming plan. Most participants took what we term a ``solution-first'' approach. This definition emphasizes ..the specific implementation of a programming pattern...

For most of our participants, a programming plan is at its core a solution. P2 defined a programming plan as \textit{``a stereotypical solution to a recurrent problem in programming.''} P3 defined programming plans as being even more specific: \textit{``A stereotypical solution to a given problem translated in a programming language.''} Whether educators believed that a programming plans should be language agnostic or not, they had a ``solution-first'' perspective where their primary focus was on the implementation of the plan.

%However, our interviewees had a variety of ways they presented this ``solution'' to learners. Approaches included code (P1, P3), pseudocode (P1), and description in natural language (P5, P6, P9). %% This shows up later

% While some participants belived that the solutions should be language agnostic, others believed that patterns were specific to the language they were implemented in.


In contrast, 
some pattern identifiers took a ``problem-first'' approach towards pattern identification. 
% Ideally we would have another sentence here explaining this perspective with more specifics. (Helping students see the underlying concepts. Helping students understand which problems should be solved in similar ways)
For these participants, a plan is \textit{``...anything that's trying to get at making these useful problem types explicit in a way that we can teach them.''} (P5). So, in this case, the focus is primarily on \textit{``analyzing what type[s] of problem[s]''} (P9) exist and then designing solutions to each problem type, which all together is referred to as a pattern.



%% Maybe we can fit in the different perspective, but right now we're skipping -KC
% However, for one of our participants, a programming pattern was a term used to describe a programming plan that was repeatedly used to achieve the same specific goal in that context. Thus, a programming plan was just a solution to a specific problem in discussion.

% \begin{quote}
%     The plan is sort of a roadmap to solve a particular problem, whereas patterns would be similarities across those plans that have been created. (P4)
% \end{quote}


% Some people include both in their definition. 

%P6 believes that one should \textit{``....Easily know how to apply the pattern.''} and thus this approach provides scaffolding for that. %Moved to usability section

%Another one of our participants also revealed that a pattern is \textit{``very individual[istic].''} (P10) %% Unsure how this fits the theme

% They added that a pattern is 
% \begin{quote}
%     .... some piece of code they are very, very used to. They know how it's structured, 
%     % so 
%     [how] it's organized, how it works. What are main mistakes that could happen with this one? (10) %% Moved to rationale section
% \end{quote}

%They also underlined that one cannot learn a pattern immediately, rather, this learning process follows a \textit{``scale from you don't know it at all and you really know this plan.''} %% Unsure how this fits the theme



%%%% Literature review

%Finally, the second author reviewed the methodology sections of all the papers in the literature search to find descriptions of the plan identification process.

%\subsection{How publications describe plan identification}

% \subsubsection{Early cognitive era (1970-1990)}

% \subsubsection{Instructional focus era (1990-2015)}

% \subsubsection{Recent era (2015-present)}



% For plan identification in new domains, a couple of our participants highlighted that 
% % talking with professionals in the domains 
% \textit{``look[ing] at what others [are doing] who are working or doing stuff in this domain''} (P8) helps give insight into \textit{``patterns that you[they] commonly think about in your[their] code''} (P4) and \textit{``what features they like to have in there''} (P8). P1 re-iterated that that it helps if \textit{``you can convince somebody to sit down with you and walk you through, pick up a representative piece of software for doing that, explaining why they're doing what they're doing''}.



% P7 encapsulated the process of familiarizing oneself with the intricacies of the domain by saying, 
% \begin{quote}
%     Doing a lot of internet searches, reading the results, and trying to distill them into a couple of paragraphs and seeing what the main ideas are. (P7)
% \end{quote}

% For self-learning, there are different places where one can look for patterns.

% \subsubsection{Example Programs}
% It is possible to look at example programs as described in the plan identification section to identify plans in a new domain. The researcher could look for repeating pieces of code and then make judgement calls to consider them as patterns or not.

% One of our interviewees also suggested, \textit{``look at APIs, libraries, and to see, because in the tutorials often they say, "Okay, this is how you should use a API or give an example.''} (P6)

% Other approaches to identify plans in a new domain using example programs includes a "problem-first" approach as described in the plan identification section where one can look at common problems existing in the domain, then for the solutions commonly used to solve that and thus create a set of candidate plans.
 

%One of our researchers highlighted that it might be useful to look at work on pattern identification in the past in that domain and hope that \textit{``someone before me had the sense to realize that there was a pattern-ish way of teaching it, and maybe then look for how did they do that?''} (P7) %% I think this is about the literature?

==> plaid-key-characteristics.tex <==

\subsection{Key Characteristics of PLAID}

PLAID supports the process of plan identification in data processing with Pandas, machine learning with Pytorch, web development using Django, and web scraping using BeautifulSoup. Advancing on the features outlined in the design artifact (Section~\ref{sec:design-artifact}) and the actions instructors performed and suggested in the design workshop, PLAID enables the following key interactions assisting instructors in refining candidates to design plans for their instruction. 


\subsubsection{Viewing Programs and Problems.}

Instructors valued the availability of code examples in condition A from our design workshop (Section~\ref{sec:design-workshop-findings}). We saw instructors scanning examples, selecting desired code pieces, and copying them over into their plan templates in all conditions in the study. Motivated to provide instructors with reference programs, PLAID provides the ``Programs (Organized by Use Case)'' tab equipping instructors with full-code programs organized in a list of short natural language descriptions of common use cases in their domain of expertise. Enabling the interactions executed by instructors in condition A, the ``Create Plan from Selection'' and ``Create Plan from Program'' buttons allow 
% < Highlight code in full code and code pane in tab1 and make a plan (D1)
% < Add a button to add full program as a plan too (D1)
users to select a part of any given code piece to create a plan \textbf{(D1)}. This interaction copies over the selected code and its respective use case into the solution and name fields, respectively. The ``Programs (Full Text)'' tab also enables viewing a list of complete code examples, allowing instructors to look at materials they would typically search for when designing plans.
% < Code explanation plugin for strange syntax (GPT) (D2)
While looking for new plans, occasionally, instructors came across syntax unfamiliar to them (e.g., due to the deprecation of old methods and the introduction of new ones like append and concat in Pandas). In this case, participants hesitated to use the suggested syntax in their plans because its functionality was unclear to them. PLAID supports a button named ``View Explanation'' where the user can select a method, function, or line of code that is unclear and click on it to understand its working \textbf{(D2)}. 
Participants also suggested being able to run code within the interface to examine the code behavior and thus mitigate the challenge of being faced with unfamiliar syntax. Thus, using PLAID, instructors are able to run complete programs to view their output \textbf{(D2)}.
% < Search in the use cases (and full progs) (D3)
Frequently, instructors relied on their expertise and experience to formulate ideas about goals for which they wanted to create plans. While interacting with condition C in the design workshop, interviewees suggested including a mechanism to search for specific keywords within code and  its natural language description. To facilitate the instructor-LLM collaboration, allowing users to find examples implementing their ideas, PLAID includes a search bar that helps users navigate the given use cases, complete programs, and effectively find specific examples they may be looking for \textbf{(D3)}.

\subsubsection{Creating Initial Candidates.}

Participants indicated difficulty mining plans from code examples (Section~\ref{sec:challenges_practice}). To alleviate these challenges, our pipeline clustered similar code examples together into plan-ful examples. The ``suggest plan'' button within PLAID presents the instructors with these plan-ful examples for refinement.
% < Keyword search/embedding filter for potential values (D1)
On clicking on any plan component fields, PLAID suggests potential values after searching its code corpus for similar examples using a keyword search \textbf{(D1)}.
% < Show use case button in solution (add highlighting) (D2)
In the design workshop, few instructors emphasized the importance of presenting worked and contextualized examples to students. To allow instructors to view suggested plans as part of a complete example, PLAID has the ‘go to a use case’ button that redirects the user to the tab with full code programs and highlights the plan as part of a complete example \textbf{(D2)}.

\subsubsection{Finalizing Plan Design.}

% From Section~\ref{sec:process_intro_plan_design}, instructors indicated drawing on their experience in the application-specific domain and instructional expertise to think about how to best solve a problem. 
In our design workshop, participants created copies of their plans to display alternative solutions to achieve the same goal, emphasizing that multiple possible solutions in code could accomplish the same goal.
% < Duplicating plans (D3)
To accelerate this process of teaching a variety of possible solutions, PLAID allows users to ``duplicate'' plans on the canvas and further edit them to present alternative solutions for the same plan \textbf{(D3)}.
% Highlight text from solution to change it to changeable areas (highlighting code itself) (D4)
In conditions A and B, instructors highlighted the changeable areas in the code itself. To allow participants to emphasize the changeable areas in code in PLAID, we implemented the ``add to changeable areas'' button. After selecting the changeable piece of code, clicking on this button highlights the text in a different color and adds it to the box of changeable areas to complete the templated plan design (\textbf{D4}).
% Grouping plans into categories (D4)
% < Multiple selection of the boxes (D4)
% < Naming groups of boxes (D4)
A handful of users postulated each plan as an example question that can be used on assessments. They intended to create multiple variants of the same question for students. They suggested that being able to visualize the different categories would be helpful. Using PLAID, users can select multiple patterns together, add them to a group, and name the group \textbf{(D4)}. 

